GRACE: Loss-Resilient Real-Time Video Communication Using Data-Scalable Autoencoder

Across many real-time video applications, we see a growing need (especially in long delays and dynamic bandwidth) to allow clients to decode each frame once any (non-empty) subset of its packets is received and improve quality with each new packet. We call it data-scalable delivery. Unfortunately, existing techniques (e.g., FEC, RS and Fountain Codes) fall short: they require either delivery of a minimum number of packets to decode frames, and/or pad video data with redundancy in anticipation of packet losses, which hurts video quality if no packets get lost. This work explores a new approach, inspired by recent advances of neural-network autoencoders, which make data-scalable delivery possible. We present Grace, a concrete data-scalable real-time video system. With the same video encoding, Grace's quality is slightly lower than traditional codec without redundancy when no packet is lost, but with each missed packet, its quality degrades much more gracefully than existing solutions, allowing clients to flexibly trade between frame delay and video quality. Grace makes two contributions: (1) it trains new custom autoencoders to balance compression efficiency and resilience against a wide range of packet losses; and (2) it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets. We test Grace (and traditional loss-resilient schemes and codecs) on real network traces and videos, and show that while Grace's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality

==> sections/abstract.tex <==
\begin{abstract}
Your abstract text goes here. Just a few facts. Whet our appetites.
Not more than 200 words, if possible, and preferably closer to 150.
\end{abstract}


==> sections/abstract_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\begin{abstract}
%Your abstract text goes here. Just a few facts. Whet our appetites.
%Not more than 200 words, if possible, and preferably closer to 150.


Across many real-time video applications, we observe an emerging need for a new primitive which allows clients to decode the next frame at a decent quality as soon as {\em any} non-empty subset of its packets is received. 
Unfortunately, today's real-time video systems fall short of this criterion, because they must reliably deliver at least certain number of packets for a frame to be decodable, and they pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which sacrifices video quality if no packets turn out lost. 
This paper articulate a new abstraction of {\em data-scalable} real-time video delivery: the {\em same} video encoding, under no packet loss, has decent quality close to traditional coding without redundancy, and {\em with each missed packet, quality naturally degrades gracefully.} 
While traditional video codecs, this paper presents the first implementation {\em autoencoder-based} data-scalable video codec and a practical real-time video system, called \name, that is built on the new video codec.
We describe the design and implementation of our custom autoencoder (NN coder and NN decoder) and a suite of frame delivering optimizations that embrace the benefit of the data-scalable primitive and can be incrementally integrated in WebRTC framework. 
\jc{a few words on result highlight}

% A growing list of applications depend on real-time video, but they face a lasting challenge---the network may delay or drop {\em any} packets, forcing the video decoder to render a frame when only a subset of its packets have arrived.
% Traditional loss-resilient approaches (FEC, fountain codes) can recover encoded data from {\em arbitrary} subset of packets, but only if the arrived data are more than the encoded data.
% So they must know, {\em before} encoding and sending a frame to the network, how many of its packets will arrive on time.
% As bursts of packet losses and delays are inevitable in wide-area networks, we argue that a more desirable solution should be {\em data-scalable}---without knowing the arrived data rate in advance, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame, and the quality should degrade gracefully if fewer packets arrive on time. 
% In this paper, we present the design and implementation of a true data-scalable real-time video system. 
% The key technique is a {\em new custom autoencoder} (a pair of NN encoder and NN decoder).
% Though traditional autoencoders are not naturally data-scalable, we can make it data-scalable by training the autoencoder to learn a smooth relationship between frame reconstruction (decoded video quality) and the amount of perturbation (packet losses) on the coded data.
% \jc{a few words on result highlight}


%Thus, it is crucial to render each frame at a high video quality without needing to wait for all packets to arrive. 
%A desirable codec, therefore, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame. 
%We refer to this seemingly simple property as {\em data-scalable} coding and argue that {\em none} of existing solutions are truly rate-scalable.
%Existing loss-resilient schemes, such as FEC and fountain codes, must know, {\em before} encoding a frame, how many packets will arrive in time. 


\end{abstract}


==> sections/abstract_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\begin{abstract}
%Your abstract text goes here. Just a few facts. Whet our appetites.
%Not more than 200 words, if possible, and preferably closer to 150.


Across many real-time video applications, we observe a growing need to allow clients to decode each frame once {\em any} (non-empty) subset of its packets is received and still obtain a high quality given the amount of data received. 
This calls for an abstraction, we refer to as {\em data-scalable} video delivery: the {\em same} video encoding, under no packet loss, has decent quality close to traditional coding without redundancy, and {\em with each missed packet, quality naturally degrades gracefully.} 
Unfortunately, existing techniques fall short of this ideal---they either must deliver at least certain number of packets for a frame to be decodable, and/or they pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost. 
We explore an alternative approach to data-scalable video delivery, using neural-network video autoencoders.
This paper presents \name, which trains a custom video autoencoder to optimizes compression efficiency {\em and} resilience to loss and transmits individually decodable packets to realize data-scalable video delivery, thus allowing clients to flexibly trade frame delay with video quality in real-time video.
\name addresses two high-level challenges: (1) how to encode and delivery real-time frames efficiently over autoencoders, and (2) how to train autoencoders to obtain decent quality under a range of packet loss rates. 
We test \name (and other traditional codecs and loss-resilient schemes) on real network traces and video datasets, and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it achieves can significantly reduce video frame delay (by 2-3$\times$ at 95th percentile) with marginally lowered video quality.

%\jc{a few words on result highlight}

%a concrete real-time video system, called \name, that is built on the new video codec.
%We describe the design and implementation of our custom autoencoder (NN coder and NN decoder) and a suite of frame delivering optimizations that embrace the benefit of the data-scalable primitive and can be incrementally integrated in WebRTC framework. 
%\jc{a few words on result highlight}

% A growing list of applications depend on real-time video, but they face a lasting challenge---the network may delay or drop {\em any} packets, forcing the video decoder to render a frame when only a subset of its packets have arrived.
% Traditional loss-resilient approaches (FEC, fountain codes) can recover encoded data from {\em arbitrary} subset of packets, but only if the arrived data are more than the encoded data.
% So they must know, {\em before} encoding and sending a frame to the network, how many of its packets will arrive on time.
% As bursts of packet losses and delays are inevitable in wide-area networks, we argue that a more desirable solution should be {\em data-scalable}---without knowing the arrived data rate in advance, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame, and the quality should degrade gracefully if fewer packets arrive on time. 
% In this paper, we present the design and implementation of a true data-scalable real-time video system. 
% The key technique is a {\em new custom autoencoder} (a pair of NN encoder and NN decoder).
% Though traditional autoencoders are not naturally data-scalable, we can make it data-scalable by training the autoencoder to learn a smooth relationship between frame reconstruction (decoded video quality) and the amount of perturbation (packet losses) on the coded data.
% \jc{a few words on result highlight}


%Thus, it is crucial to render each frame at a high video quality without needing to wait for all packets to arrive. 
%A desirable codec, therefore, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame. 
%We refer to this seemingly simple property as {\em data-scalable} coding and argue that {\em none} of existing solutions are truly rate-scalable.
%Existing loss-resilient schemes, such as FEC and fountain codes, must know, {\em before} encoding a frame, how many packets will arrive in time. 


\end{abstract}


==> sections/eval.tex <==
\tightsection{Evaluation}

\tightsubsection{Experiment setup}
\begin{itemize}
    \item Testbed (simulation & emulation)
    \item Traces we used
    \item Baselines
\end{itemize}

\tightsubsection{Simulation (frame level)}
Frame level quality improvement compared with baselines
\begin{itemize}
    \item PSNR under different losses
    \item PSNR CDF for different frames (we have a better tail)
\end{itemize}

\tightsubsection{Trace-driven experiments (packet level)}
\begin{itemize}
    \item tail PSNR v.s. avg delay
    \item avg PSNR v.s. tail delay
\end{itemize}

\tightsubsection{Microbenchmark}
\begin{itemize}
    \item Improvement on different video type
    \item Improvement breakdown
\end{itemize}

==> sections/eval_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Evaluation}
\label{sec:eval}

The findings from our evaluation of \name can be summarized as follows:
\begin{packeditemize}
\item Though in terms of quality under no packet loss, \newae is on par with H.264 and slightly worse than H.265, it is data-scalable---graceful quality degradation with higher loss rate---under various video content and bitrate. 
\jc{a few example numbers}
\item Under dynamic network conditions, \name strikes a better trade-off between average video quality and tail delay than a wide range of baselines.
\jc{a few example numbers}
\end{packeditemize}

\subsection{Setup}

We test \name's implementation (described in \S\ref{??}) at two levels.
First, we test \newae's loss resilience when encoding/decoding real videos under controlled packet losses, and compare it with other loss-resilient schemes.
Second, we test \name (including its codec and delivery framework) over real bandwidth traces, and compare it with other real-time baseline solutions (baselines explained shortly).



\mypara{Network and compute conditions}
We test \name on \fillme real bandwidth traces from FCC.
We filter traces \fillme.\jc{ziyi and hanchen, please describe the filter here.}

We conduct all experiments on a machine with two Nvidia \fillme GPUs as the sender and receiver (each using one GPU). 
\jc{more details, such as cuda version, linux version, cpu, memory, etc}
To make the results more convincing, we measure \name's encoding and decoding delays on the GPU (see results in \S\ref{??}) and we include these delays in \name's frame delay. 

Our evaluation uses videos from three datasets (\fillme, \fillme and \fillme), each video is of \fillme minutes. 
The videos cover three resolutions (360p at 25fps, 720p at 25fps, and 1080p at 20fps), with at least \fillme videos in each resolution. 
The performance is reported as an average across all the frames in the videos.


\mypara{Baselines}
We compare the performance of \name with multiple state-of-the-art real-time video techniques that use different combinations of video coding and congestion control algorithms: 
\begin{packeditemize}
\item {\em Reference:} H.26x with adaptive FEC and GCC
\item {\em Salsify:}
\item {\em Idealized SVC:}
\end{packeditemize}


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/psnr-bpp-example.pdf}
         \label{fig:}
    \caption{an example. need more of it in different datasets}
    \label{fig:}
\end{figure}


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-kin.pdf}
         \caption{Kinetics dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-uvg.pdf}
         \caption{UVG dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-fvc.pdf}
         \caption{FVC dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \caption{PSNR vs LOSS different dataset (bpp = 0.08)}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-lowbr.pdf}
         \caption{Small bitrate (bpp = 0.08)}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-medbr.pdf}
         \caption{Med bitrate (bpp = 0.16)}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-highbr.pdf}
         \caption{High bitrates (bpp = 0.24)}
         \label{fig:}
     \end{subfigure}
    \caption{PSNR vs LOSS of different bitrate, using multiple datasets}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-kin.pdf}
         \caption{Kinetics dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-uvg.pdf}
         \caption{UVG dataset }
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-fvc.pdf}
         \caption{FVC dataset}
         \label{fig:}
     \end{subfigure}
    \caption{PSNR vs BPP different dataset}
    \label{fig:}
\end{figure*}

\subsection{Loss resilience}

\jc{
\begin{itemize}
    \item by bitrate
    \item by video set
    \item psnr vs. bitrate
\end{itemize}
}



\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
    \caption{Aggressiveness = 1}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
    \caption{Aggressiveness = 5}
    \label{fig:}
\end{figure*}


\begin{figure}[t!]
    \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/loss-distribution.pdf}
         \caption{Impact of different data loss distribution used during training}
         \label{fig:training_loss_distribution}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/loss-pattern.pdf}
         \caption{Impact of different data loss pattern used during training}
         \label{fig:training_loss_pattern}
     \end{subfigure}
    \label{fig:training_loss_simulation}
\end{figure}

\subsection{Video quality vs. tail delay}

\jc{
\begin{itemize}
    \item by trace set
    \item by rtt
    \item by queue length
    \item a concrete example
\end{itemize}
}

\subsection{Memory and compute overhead}

\jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}


\subsection{Design choices in \name}

\jc{
\begin{itemize}
    \item different training loss patterns
    \item different training \rate distributions
    \item saliency-based redunancy
    \item packet prioritization
    \item computing overhead in delay and in memory
\end{itemize}
}



==> sections/intro.tex <==
%-------------------------------------------------------------------------------
\tightsection{Introduction}
%-------------------------------------------------------------------------------

Usage of real-time video conferencing applications are increasing rapidly.

The goal of real time video conferencing is high visual quality and low latency. However, achieving such goal is challenging because of unavoidable and unpredictable packet losses.

Towards this problem, state-of-art solutions can be divided into 2 categories: retransmission-based method and hand-crafted loss tolerant mechanisms. However, all of those methods are not optimal...

Our goal and our design...

==> sections/intro_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Introduction}

Real-time video traffic is now on par with traditional streaming videos, with applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{see refs from hotnets}.
Video in Chrome over WebRTC grew 100x during 2020~\cite{??}, and one global industry survey found that services based on real-time videos grew from less than 5\% to over 28\% between 2020 and 2021~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

With the unprecedented proliferation of real-time video, we see an emerging need for the ability to render a frame with {\em high quality} as soon as {\em any} non-empty subset of its packets is received.
The flexibility for clients to {\em balance frame-level delay and rendering quality} is particularly useful under {\em long RTT} (\eg long enough to render retransmission ineffective), and {\em intermittent} packet drops, delays or reordering, caused by bursty cross-traffic and natural variation of encoded frame sizes.\footnote{This problem so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{report}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{??}).}

\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:intro-example}
\end{figure}

Unfortunately, current loss-resilient schemes fall short of this expectation, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 
For instance, FEC, the loss-resilient method ubiquitously used in WebRTC, requires a certain fraction of packets be reliably received before a frame is decodable. 
Moreover, to tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
Setting an appropriate level of redundancy is, however, well-known to be hard under high packet jitters~\cite{??}---too much redundancy causes underutilization of bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy forces the receiver to wait for (or resend) more packets. 
Figure~\ref{fig:intro-example} illustrates this tradeoff: the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
Like FEC, other schemes (\eg SVC, intra-MB insertion) also must reliably deliver at least certain number of packets and add redundancy that sacrifices video quality if no packets are delayed/lost (\S\ref{??}).




We argue that a better video codec should be {\em data scalable}, which entails three requirements: 
(1) the coding of a video frame only depends on target bitrate (not predicted loss rate), 
(2) the frame is decodable once {\em any} non-empty subset of its packets are received and the decoded quality improves with more packets received, and 
(3) for any x\%, the decoded quality with x\% arrived packets is close to the classic codec (like H.265) with x\% FEC redundancy.\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality ideally is proportional to throughput. Unfortunately, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. 
In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
In contrast to existing codec (including loss-resilient ones), a data-salable codec eschews the need for the sender to inject redundancy based on predicted packet jitter/losses and allows the receiver to flexibly choose when to decode a frame once one of its packets arrives while still enjoying decent video quality.


\begin{comment}

Unlike FEC which sets redundancy rate {\em before} sending data out, our goal is to encode a frame in a \rate-agnostic way and decode the frame under any \rate (less than 100\%) at a similar quality as current FEC-based coding {\em if} it knew \rate. 
In other words, 
(1) under zero \rate, the decoded video quality should be close to that of existing video coding without FEC redundancy, and 
(2) the decoded video quality should degrade gracefully with higher \rate, with a similar quality as FEC-based coding if FEC knows the \rate. 
% So without knowing \rate, it should achieve similar quality as existing real-time video systems when they know \rate. 
In short, the envisioned real-time video system eschews the need for \rate prediction.

\end{comment}


Achieving data-scalable coding is clearly a daunting task, but this paper demonstrates that it is possible. 
We explore a new approach to data-scalable codec, by borrowing and customizing the emergent deep autoencoders, a class of neural-network coder/decoders that compress multimedia data (videos and images) highly efficiently. 
Though existing autoencoders do not tolerate loss, we show that by letting them ``experience'' different rates of packet loss during training, we can create {\em data-scalable autoencoders} learn not only how to code video pixels efficiently but also how to code them in a way that is resilient to missing packets.
% Training in itself is not straightforward, since packet losses are not naturally differentiable.
While the idea of data-scalable autoencoder is arguably simple, its performance gain is quite remarkable. 
Figure~\ref{fig:intro-example} contrasts the performance of an example data-scalable autoencoder with prior loss-resilient schemes. 

Our goal is {\em not} merely showing that data-scalable autoencoders are possible. 
Instead, our main contribution is to explore key questions regarding {\em how to develop and use data-scalable autoencoders in real-time video systems} in the context of \name, a concrete system based on data-scalable autoencoders. 
These questions include
why an autoencoder could be resilient to packet losses, 
how to best incorporate packet losses in autoencoder training (given packet loss is not naturally differentiable), and
how well an autoencoder fares in unseen content {\em and} unseen \rates. 
Moreover, since the video codec is tightly connected to other components in a real-time video system, data-scalable autoencoders bring up unique design questions, such as 
how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 

% This begs several immediate and critical questions.

% Instead, we try to answer these technical questions in the context of \name, a concrete system based on data-scalable autoencoders. 


% To best utilize data-scalable autoencoders in practice, they should also be  video streaming system. 


Though the concept of autoencoders has been used in video streaming~\cite{??} and image compression in wireless communication~\cite{??}, to our best knowledge, these questions have not been systematically studied.
For instance, \fillme \jc{pick one or two exciting technical contributions}



Our evaluation shows \jc{eval highlights}

\jc{outline the roadmap and highlight the contribution again}

\jc{need a forward pointer to 2.2 (caveats of autoencoders)}




==> sections/intro_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Introduction}

Real-time video traffic is on par with traditional streaming videos. 
With applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{see refs from hotnets}, video in Chrome over WebRTC grew 100x during 2020~\cite{??}, and one global industry survey found that services based on real-time videos grew from less than 5\% to over 28\% between 2020 and 2021~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

With the unprecedented proliferation, real-time video applications are expected to operate in not only low-RTT and largely stable networks, but over connections with {\em long RTT} (which renders retransmission ineffective) or {\em high packet jitters} and {\em intermittent losses} (which makes accurate rate adaptation difficult).\footnote{This problem so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{report}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{??}).}
For instance, retransmitting a packet along a path with 100ms RTT will delay or skip at least three frames in a 25fps video stream (a new frame every 40ms).
Prior measurements have confirmed that such long RTT is common in video conferencing and that high packet jitters and losses are not rare, due to various reasons such as bursty cross-traffic, packet reordering, and variation of encoded frame sizes.\jc{the last sentence should be replaced with numbers cited from recent papers}

%\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        \includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss.pdf}
         \label{fig:}
    \caption{Loss resilience comparison among different schemes. The encoding bitrate is set at \fillme Mbps. 
    More results can be found in \S\ref{sec:eval}.\jc{YIHUA, remember to add a line of 264 without loss.}}
    \label{fig:intro-example}
\end{figure}

Thus, to flexibly trade between video quality and video delay (without skipping frames), a client should ideally be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
Unfortunately, existing loss-resilient schemes fall short of this expectation.
%, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 
For instance, Forward Error Correction (FEC) is ubiquitously used in WebRTC, and it requires a certain fraction of packets be reliably received before a frame is decodable. 
To tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
Thus, choosing an appropriate level of redundancy is known to be difficult under high packet jitters~\cite{??}.
As illustrated in Figure~\ref{fig:intro-example}, too much redundancy would underutilize bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy would drive the receiver to wait for (or resend) more packets. 
In short, the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
As elaborated in \S\ref{??}, other schemes (\eg SVC, inter-MB insertion) also must deliver at least certain number of packets for a frame to be decodable, and/or pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost.

To address these limitations, we advocate for a new abstraction, referred to as {\em data-scalable} video delivery, which entails two requirements: 
(1) the coding of a video frame does not depend on an anticipated loss rate, 
(2) a frame is decodable once {\em any} non-empty subset of its packets are received and the decoded quality improves with more packets received.\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality increase with throughput. However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
In other words, the decoded video quality, under no packet losses, should be similar to a classic codecs (\eg H.264, H.265) and degrade {\em gracefully} with more lost packets. 
In essence, the abstraction of data-salable video delivery eschews the need for the sender to inject redundancy based on predicted packet losses and instead allows the receiver to flexibly choose when to decode a frame once any its packets have arrived while enjoying decent video quality.


\begin{comment}

Unlike FEC which sets redundancy rate {\em before} sending data out, our goal is to encode a frame in a \rate-agnostic way and decode the frame under any \rate (less than 100\%) at a similar quality as current FEC-based coding {\em if} it knew \rate. 
In other words, 
(1) under zero \rate, the decoded video quality should be close to that of existing video coding without FEC redundancy, and 
(2) the decoded video quality should degrade gracefully with higher \rate, with a similar quality as FEC-based coding if FEC knows the \rate. 
% So without knowing \rate, it should achieve similar quality as existing real-time video systems when they know \rate. 
In short, the envisioned real-time video system eschews the need for \rate prediction.

\end{comment}


%While data-scalable coding might be possible with existing codecs, we
We explore a new approach to data-scalable coding, by borrowing and customizing the emergent neural-net autoencoders, a class of neural-network coder/decoders for multimedia data (videos and images). 
Existing autoencoders are developed with compression efficiency as the objective, but we show that by injecting emulated packet losses during autoencoder training, we can create a {\em data-scalable autoencoders}, that learn not only how to code video pixels efficiently but also how to code them in a way that is resilient to missing packets.
% Training in itself is not straightforward, since packet losses are not naturally differentiable.
%While the idea of data-scalable autoencoder is arguably simple, its performance gain is quite remarkable. 
The resulting autoencoder, though slightly less efficient at compressing videos under no packet losses than classic heavily engineered codecs, can meet the two criteria of data-scalable coding. 
Figure~\ref{fig:intro-example} shows an example result: the decoded quality at x\% packet losses should be close to that of H.264 or H.265 with x\% FEC redundancy, which can be viewed as a reference design that optimizes compression efficiency, not loss resilience.

Besides the possibility of data-scalable autoencoders, we also present the design and implementation of \name, a concrete real-time video system.
\name tackles two high-level challenges. 

First, how to train a data-scalable autoencoder to tolerate various unseen packet loss rates. 
This challenge entails several subquestions: 
how packet losses should be emulated as part of model training given that the impact of packet loss on coded data is non-differentiable, 
what packet losses should be revealed to the autoencoder during training, 
and why our autoencoder is more resilient to data losses than existing schemes.

Second, how to realize data-scalable delivery over data generated by the data-scalable autoencoder. 
This involves several design questions such as how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 
Moreover, since use of autoencoders in real-time video delivery is relatively new, we also examine various strategies for bitrate adaptation and key frame insertion in the context of \name.

No individual component of \name is particularly intricate, and some are inspired by prior work. 
However, the contribution of \name lies in an end-to-end real-time video delivery framework, which tackles various challenges arising from training data-scalable autoencoder and delivering autoenocer output data.


%\jc{there's some concerns regarding autoencoders. these questions are answered for the first time}

%how to best emulate packet losses during training so that the resulting autoencoder can handle and
%how well an autoencoder fares in unseen content {\em and} unseen \rates. 
%Moreover, since the video codec is tightly connected to other components in a real-time video system, data-scalable autoencoders bring up unique design questions, such as 
%how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 

% This begs several immediate and critical questions.

% Instead, we try to answer these technical questions in the context of \name, a concrete system based on data-scalable autoencoders. 


% To best utilize data-scalable autoencoders in practice, they should also be  video streaming system. 


Admittedly, we are not the first to use autoencoders in video compression. 
Applications of autoencoders can be found in wireless and data communication to compress images, video files, and signals~\cite{??}, and notably a recent work uses custom autoencoders to obtain highly efficient scalable video coding (SVC). 
However, to our best knowledge, \name is the first to use custom autoencoders to realize data-scalable video delivery.



Our evaluation shows \jc{eval highlights}

\jc{outline the roadmap and highlight the contribution again}

\jc{need a forward pointer to 2.2 (caveats of autoencoders)}

\jc{
\begin{itemize}
    \item content generalization
    \item clarify the use cases
    \item putting the improvement into context
    \item 
\end{itemize}
}





==> sections/intro_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Introduction}

Real-time videos are as important and popular as traditional streaming videos. 
With applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{webrtc-gaming-1,webrtc-gaming-2,webrtc-vr-1,webrtc-vr-2,webrtc-iot-1,webrtc-iot-2}, video in Chrome over WebRTC grew 100x during 2020~\cite{blum2021webrtc}, and one global industry survey found that services based on real-time videos grew from less than 5\% to over 28\% between 2020 and 2021~\cite{video-report-2020,video-report-2021}.
% ~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

With users increasingly depending on real-time videos, it is crucial to deliver video frames smoothly and with decent quality under a wide range of network conditions\footnote{This problem so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{report}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{??}).}, including
long latency and highly dynamic network jitters, causing intermittent bursts of {\em packet losses}. 
Importantly, in real-time video, packet losses include {\bf not only} randomly dropped packets, but also those delayed (due to congestion, path fluctuation, or retransmission) and thus arriving after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps)\footnote{In lack of a better term, we call them {\em packet losses}.}.
%{\em long latency}, {\em high packet jitters} and {\em intermittent bursts of packet losses}.
%Importantly, in real-time video, packet losses include {\bf not only} randomly dropped packets, but also those delayed by congestion, path fluctuation, or retransmission and arriving after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps)\footnote{In lack of a better term, we call them {\em packet losses}.}.
Recent measurements shown that high packet jitters and losses are not rare in real-time video applications~\cite{jansen2018performance,concerto}; \eg a drop of bandwidth from 3Mbps to 500Kbps can make 75\% of packets missing their playback time and raise the RTT by 6$\times$.
%one study found that in \fillme sessions, packet loss rates can be up-to \fillme\% for \fillme\% frames.\jc{YIHUA, please fill the numbers}
Retransmission is often too late with long RTT, since the jitter buffer is only \fillme; \eg resending packets on a path with 100ms RTT will delay or skip at least three frames in a 25fps video stream (\ie a new frame every 40ms).

\begin{comment}
Since real-time video clients have a very shallow jitter buffer (\fillme), a packet is effectively lost as long as it is delayed long enough (due to retransmission, congestion, path fluctuation, etc) to affect the decoding of a frame (and subsequent frames).\footnote{It is important that in real-time video, packet losses {\bf not only} include packets randomly dropped by the network, but also those that are delayed due to congestion, path fluctuation, or retransmission and arrive later than when the frame it belongs to is supposed to be decoded (\eg 40ms after the last frame was decoded if the video is 25fps). In lack of a better term, we call them packet losses, and the packet loss rates can thus easily be as high as \fillme\%, as shown in recent measurements~\cite{??,??}}
For instance, retransmitting packets on a path with 100ms RTT could delay (or skip) at least three frames in a 25fps video stream (\ie a new frame every 40ms).
Prior measurements have confirmed that such long RTT is common in video conferencing and that high packet jitters and losses are not rare, due to reasons including bursty cross-traffic, packet reordering, and variation of encoded frame sizes.
\end{comment}

%\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        \includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss.pdf}
         \label{fig:}
    \caption{Comparing different loss-resilient schemes when the actual encoding bitrate is set at \fillme Mbps. 
    Quality of \name's autoencoder achieves a smoother quality degradation as packet loss rate increases.
    More results can be found in \S\ref{sec:eval}.\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}}
    \label{fig:intro-example}
\end{figure}

%To flexibly balance video quality and video delay, ideally a client should be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
Many prior techniques have been proposed to tolerate packet losses, but they still require retransmission or trade low quality for higher loss resilience. 
%
%An ideal client should therefore tolerate packet losses be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
%Unfortunately, existing loss-resilient schemes fall short of this expectation.
%, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 
For instance, Forward Error Correction (FEC) requires a minimum fraction of packets be reliably received before a frame is decodable, and to lower this minimum fraction, more redundancy must be added, forcing the sender to encode a frame in lower quality before sending the packets out. 
As a result (illustrated in Figure~\ref{fig:intro-example}), video quality will be low if packet losses are overestimated, or delay will be high if packet losses are underestimated. 
Similar tradeoffs between quality and delay (loss resilience) manifest themselves in other schemes (\eg SVC, inter-MB insertion) as well (\S\ref{subsec:abstractions}). 

%To tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
%Thus, choosing an appropriate level of redundancy is known to be difficult under high packet jitters~\cite{??}.
%As illustrated in Figure~\ref{fig:intro-example}, too much redundancy would underutilize bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy would drive the receiver to wait for (or resend) more packets. 
%In short, the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
%As elaborated in \S\ref{??}, other schemes (\eg SVC, inter-MB insertion) also must deliver at least certain number of packets for a frame to be decodable, and/or pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost.

To address these limitations, we advocate for a new abstraction, referred to as {\em data-scalable} video delivery, and a practical implementation of it: the same encoding of a frame can be decodable once {\em any} non-empty subset of its packets are received (as opposed to a minimum set of packets as in FEC, RS or fountain codes) and achieve higher quality with each new packet received.\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality increase with throughput. However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
%, which entails two requirements: 
%(1) the coding of a video frame does not depend on an anticipated loss rate, 
%(2) a frame is decodable once {\em any} non-empty subset of its packets are received and the decoded quality improves with more packets received.
%In other words, the decoded video quality degrades {\em gracefully} with more lost packets. 
In other words, a frame is decoded at a similar quality to a classic codecs (\eg H.26x) when no packet is lost, and the quality degrades {\em gracefully} with more lost packets. 
%the decoded video quality, under no packet losses, should be similar to a classic codecs (\eg H.264, H.265) and degrade {\em gracefully} with more lost packets. 
The abstraction of data-salable delivery therefore does not need to predict packet losses before sending video packets; instead, the receiver can flexibly choose when to decode a frame once any packets have arrived while enjoying decent video quality.

%the sender to inject redundancy based on predicted packet losses; 


\begin{comment}

Unlike FEC which sets redundancy rate {\em before} sending data out, our goal is to encode a frame in a \rate-agnostic way and decode the frame under any \rate (less than 100\%) at a similar quality as current FEC-based coding {\em if} it knew \rate. 
In other words, 
(1) under zero \rate, the decoded video quality should be close to that of existing video coding without FEC redundancy, and 
(2) the decoded video quality should degrade gracefully with higher \rate, with a similar quality as FEC-based coding if FEC knows the \rate. 
% So without knowing \rate, it should achieve similar quality as existing real-time video systems when they know \rate. 
In short, the envisioned real-time video system eschews the need for \rate prediction.

\end{comment}

We explore a new approach to data-scalable delivery, inspired by the emergent neural {\em autoencoders}.
We discuss the benefits and caveats of using autoencoders in \S\ref{subsec:why-autoencoder}.
%, neural-network coder/decoders for multimedia data (videos and images). 
Thanks to their neural-network architecture, autoencoder {\em could} be data-scalable, but existing autoencoders' quality drops quite quickly with lost packets.
We show, however, that by simulating packet losses during autoencoder training, we can train {\em data-scalable autoencoders}, that learn not only how to compress video pixels efficiently but also how to code them in ways resilient to missing packets.

%While data-scalable coding might be possible with existing codecs, we
%This paper explores a new approach to data-scalable coding, by borrowing and customizing autoencoders, an emergent class of neural-net coder/decoders for multimedia data (videos and images). 
%Existing autoencoders are developed with compression efficiency as the objective, but we show that by injecting emulated packet losses during autoencoder training, we can create a {\em data-scalable autoencoders}, that learn not only how to code video pixels efficiently but also how to code them in a way that is resilient to missing packets.
%% Training in itself is not straightforward, since packet losses are not naturally differentiable.
%%While the idea of data-scalable autoencoder is arguably simple, its performance gain is quite remarkable. 
%The resulting autoencoder, though slightly less efficient at compressing videos under no packet losses than classic heavily engineered codecs, can meet the two criteria of data-scalable coding. 
%Figure~\ref{fig:intro-example} shows an example result: the decoded quality at x\% packet losses should be close to that of H.264 or H.265 with x\% FEC redundancy, which can be viewed as a reference design that optimizes compression efficiency, not loss resilience.

This work presents the design and implementation of \name, a concrete real-time video system based on data-scalable autoencoders. 
%To make data-scalable autoencoders practical, we present the design and implementation of \name, an end-to-end real-time video system.
Figure~\ref{fig:intro-example} shows an example result: its quality degrades gracefully with more packet losses, and at various packet loss rate, its quality is comparable to that of H.264 or H.265 with adequate FEC redundancy. 
%, which can be viewed as a traditional reference that optimizes compression efficiency and loss resilience.

%the decoded quality at x\% packet losses is close to that of H.264 or H.265 with x\% FEC redundancy, which can be viewed as a reference design that optimizes compression efficiency, but not loss resilience.

\name tackles two high-level challenges. 
First, how to train data-scalable autoencoders (\S\ref{sec:training}). 
We discuss design choices regarding how packet losses should be simulated as part of model training given that the impact of packet loss on coded data is non-differentiable, and
what packet losses should be revealed during autoencoder training in order to balance quality at high rates and low rates of packet losses.
We also discuss why autoencoders can be made data-scalable.


%First, how to train a data-scalable autoencoder to tolerate various unseen packet loss rates. 
%This challenge entails several subquestions, such as
%how packet losses should be simulated as part of model training given that the impact of packet loss on coded data is non-differentiable, and
%what packet losses should be revealed during autoencoder training in order to balance quality at high rates and low rates of packet losses.

%and why our autoencoder is more resilient to data losses than existing schemes.

Second, how video frames encoded by autoencoder should be streamed to realize data scalable delivery over a {\em sequence} of frames. 
\name uses custom strategies of packetization and frame scheduling, such that the (individually decodable) packets are received and decoded in a way that balances frame delay  and quality (\S\ref{sec:delivery}).
\name also provides optimizations to adapt bitrate on top of autoencoders and reduce compute and memory overheads (\S\ref{subsec:optimize}).
\name is {\em complementary} to congestion control which decides how fast packets should be sent, while \name decides {\em what} packets should be send.

%Second, how to realize data-scalable delivery over data generated by the data-scalable autoencoder. 
%This involves several design questions such as how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 
%Moreover, since use of autoencoders in real-time video delivery is relatively new, we also examine various strategies for bitrate adaptation and key frame insertion in the context of \name.

%Most components of \name are inspired by prior work.
%No individual component of \name is particularly new. %, and some are inspired by prior work. 



%\jc{there's some concerns regarding autoencoders. these questions are answered for the first time}

%how to best emulate packet losses during training so that the resulting autoencoder can handle and
%how well an autoencoder fares in unseen content {\em and} unseen \rates. 
%Moreover, since the video codec is tightly connected to other components in a real-time video system, data-scalable autoencoders bring up unique design questions, such as 
%how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 

% This begs several immediate and critical questions.

% Instead, we try to answer these technical questions in the context of \name, a concrete system based on data-scalable autoencoders. 


% To best utilize data-scalable autoencoders in practice, they should also be  video streaming system. 



Importantly, \name does {\em not} improve coding efficiency (higher quality with less bits), which most heavily engineered video codecs strive to optimize. 
In fact, \name's video quality is slightly lower than H.265 at same bitrate. 
However, \name enables data-scalable delivery to achieve better quality with lower delay in high jitter networks.


We are not the first to use autoencoders in video compression. 
Applications of autoencoders can be found in wireless and data communication to compress images, video files, and signals~\cite{erpek2020deep}, and notably a recent work uses custom autoencoders to obtain highly efficient scalable video coding (SVC)~\cite{swift}. 
%Many aspects of \name are also inspired by prior work. 
That said, \name, to our best knowledge, is the first to use custom autoencoders to realize data-scalable video delivery.
The contribution of \name is an end-to-end real-time video delivery framework, which tackles various challenges arising from training and using data-scalable autoencoder in real-time video communication.



We test \name and traditional loss-resilient schemes and codecs on real and synthetic network traces, as well as various genres of videos.
Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces video frame delay (by 2-3$\times$ at the 95th percentile) with marginally lowered video quality (less than \fillme~dB in SSIM).
To put it in perspective, \name significantly improves playback smoothness (\fillme less stalls with a jitter buffer) and reduces the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing).

\textbf{This work does not raise any ethical issues.}

%\jc{eval highlights}

%\jc{outline the roadmap and highlight the contribution again}

%\jc{need a forward pointer to 2.2 (caveats of autoencoders)}
%
%\jc{
%\begin{itemize}
%    \item content generalization
%    \item clarify the use cases
%    \item putting the improvement into context
%    \item 
%\end{itemize}
%}





==> sections/motivate_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Background}



% Real-time video, it is crucial that enough data is timely received for each frame, so that the high-quality frames can be rendered at a fixed interval (\eg every 50ms for 20fps). 
% However, as most packet networks have occasional congestion, delay jitter and packet losses, not all packets of a frame may arrive timely.
% Retransmitting missing packets is also inefficient if the round trip time is long.
% Therefore, loss-resilient schemes are required to ensure that a frame can be decoded at a high quality even if a fraction of its packets have not arrived when it is supposed to be decoded, \ie non-zero deadline-missing rate or \rate. 



\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.85\linewidth]{figs/motivate_example_placeholder.pdf}
         \label{fig:}
    \caption{}
    \label{fig:motivate-example}
\end{figure}

\subsection{Prior Loss-Resilient Schemes}


With occasional congestion and packet jitter and losses in most packet networks, it is desirable that a real-time video client can decode and render the next frame as soon as a subset of its packets are received.
Therefore, loss-resilient techniques have seen intensive research for over two decades, despite that other types of streaming videos (YouTube, Netfliex) have long become TCP-based. 

\mypara{Forward error correction (FEC)}
We start with FEC as it is the most widely used loss-resilient scheme in today's real-time video systems (mostly WebRTC-based). 
(Other loss-resilient schemes (\fillme) will be discussed shortly.)
Put simply, an optimal FEC takes any file of size $M$ bytes, codes it with redundancy bits, and sends the coded data out.
The receiver can then decode the coded data as long as {\em any} $M$ bytes are received. 
Fountain code is a variant of FEC that does not limit the size of the coded data, so the sender can send as many bytes as it wants, and the receiver can decode it once $M$ bytes have arrive. 
Readers can refer to~\cite{??,??} for a more in-depth introduction of FEC.
FEC has been studied intensively in the IEEE multimedia community, with \fillme and \fillme achieving near-ideal performance of FEC and fountain codes.
For simplicity, this paper assumes ideal FEC (\ie the coded data generated from $M$ bytes is decodable once any $M$ bytes are received)\footnote{\jc{a footnote on the suboptimal use of fec in webrtc}}.


FEC is known to have the ``cliff effect'': for a given data (a frame or chunk encoded by a video coder like H.265), no matter how FEC adds redundancy, at least as many bytes as in the original data must be delivered.
And since the decoded video quality remains the same even if more bytes arrive (Figure~\ref{fig:intro-example}), the video coder should encode the video at the highest sustainable bitrate. 
If we know that under the sending rate of $c$, $r$ fraction of data will not arrive timely (\eg when a frame should be rendered), then ideally, the video should be encoded at bitrate $c\cdot(1-r)$ and sent with redundancy rate $r$. 
With less redundancy, the receiver must wait longer for more packets to arrive or retransmit; with more redundancy, the video bitrate will be lowered.
Thus, {\em FEC will be most effective {\bf if} the sender knows how many bytes can be timely delivered in advance.} 
% For a link of 4Mbps and negligible RTT, to deliver a frame within 100ms, the ideal frame size cannot exceed 50KB; otherwise, no matter how FEC adds redundancy, it always takes longer than 100ms for FEC to get enough bytes to decode the frame. 
% To see why this may be problematic, consider streaming a video of 20fps over a hypothetical network connection of 5Mbps (with zero RTT). 
% over a link of 4Mbps and negligible RTT, no matter how FEC adds redundancy, it will always take about one second to deliver 200KB of data required for FEC to recreate the frame data. 
% Otherwise, the frame has to be skipped, and the last decoded frame will fill in, causing degraded visual quality\jc{need a citation or some justification}. 
% To pick an appropriate redundancy rate, FEC-based loss-resilient schemes have developed various algorithms to predict future \rate based on history network conditions and current sending rate (\eg~\cite{??,??,??}). 
% , in order to determine how fast data should be sent out ($c$) and how much redundancy should be introduced ($r$), such that $c\cdot(1-r)$ matches the receiving data rate at the receiver.
Despite many efforts to predict packet loss rate, pick a desirable redundancy rate before knowing the future \rate is hard, especially
% But since $r$ is picked {\em before} the data is sent, it is hard to always pick a desirable \rate, 
if \rate changes dynamically and non-stationarily in packet networks.\footnote{In fairness, FEC is effective at concealing random packet losses in wireless channels with a largely stable erasure rate.
Moreover, the FEC redundancy can help the sender to quickly probe bandwidth~\cite{??}.}



% Given a target sending rate $w$ decided by a congestion control logic, if the estimated \rate (the fraction of data not arriving by the time decoder wishes to decodes the data) is $r$, a video frame will be compressed by a video encoder at a bitrate $b=w\cdot(1-r)$ and then coded by FEC with redundancy of $c\cdot r$.
% An adaptive logic is then needed to determine the FEC redundancy rate (\eg~\cite{??,??,??}).
% % This is feasible when the \rate $r$ for a sending rate $w$ is reliably estimated, but 
% However, \rate often changes dynamically and non-stationarily in packet networks.

\jc{an example figure of dmr over time here, with fec logic}

Figure~\ref{??} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a bandwidth trace sample from \fillme over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate cannot adjust timely, causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if we let FEC adapt more conservatively (\eg increase redundancy faster but decrease it more slowly), as shown \fillme. But this is at the cost of much lower video quality, as more bytes are used for redundancy.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.

\jc{mention the findings corroborate with \cite{\url{https://docs.google.com/document/d/1Hg1SaLEl6T4rEU9j-isovCo8VEjjnuCPTcLNJewj7Nk/edit}}}


\jc{need a figure here to clarify different between video coder and fec coder}

\mypara{Loss-resilient video coding}
In addition to FEC (and other channel-coding schemes), prior work has also studied loss-resilient video coding techniques, which add redundancy during the video codec (\eg H.265) rather than after. 
These schemes are usually called ``source coding'' in the multimedia literature.
For instance, \jc{explain R/D optimization, unequal protection, and dynamic reference selection}




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.6\linewidth]{figs/motivate_regime.pdf}
         \label{fig:}
    \caption{}
    \label{fig:motivate-regime}
\end{figure}


\mypara{Compression efficiency vs. loss resilience}
Both FEC-based schemes and loss-resilient video coding face a fundamental limitation:
compared to traditional coder (\eg H.265) that are optimized for video coding efficiency (less bits for higher quality), these loss-resilient coders are less efficient in that they use more bits (\ie redundancy) to obtain same quality in the absence of any packet loss (\ie zero \rate).
In other words, they must trade compression efficiency for loss resilience, so the rate of redundancy is highly sensitive to \rate prediction. 
\jc{a few more examples on how various video coders trades compression efficiency for loss resilience}



\jc{add a figure of unpredictable dmr vs long delay}

Figure~\ref{fig:??} illustrates when existing schemes are effective.
When the RTT of the connection is low compared to the desirable frame delay, packet retransmission would be sufficient to conceal any packet losses.
When the \rate of the next frame is stationary or largely predictable, FEC-based schemes will be sufficient. However, current solutions will fall short in the case of high RTT and highly dynamic \rates.



Connections with dynamic \rates and high RTT are not rare in practice. 
For instance, we can run a ``what-if'' analysis over the trace of Figure~\ref{??} to reveal the \rate of each frame if a maximum frame delay of \fillme is imposed. 
We keep the same congestion control logic and measure how much data of each frame arrive at the receiver after the maximum frame delay. 
We see \rate varies just as much as the frame delays, especially when bandwidth suddenly drops.
It is not surprise then that existing FEC logic in WebRTC cannot always set an appropriate FEC redundancy rate that is high enough to maintain a low tail frame delay, but not too high to sacrifice video bitrate.
% if a frame has a \rate of 30\%, the optimal FEC redundancy rates would have been 30\% (\ie video encoding bitrate is 70\% of the sending rate, if such encoding is available). 
% We can see that the optimal redundancy rates can be just as highly dynamic as the frame delays.


In summary, existing loss-resilient schemes encode video based on estimated \rate and are most effective only when the estimation is accurate. 
Overestimation leads to too much redundancy and low video quality, but underestimation cause more retransmission and video frame delays.



\subsection{Autoencoders}


This work is framework built on autoencoders, an emergent class of learned coders for video frames, including I-frames and P-frames.
Compared to early autoencoder variants, recent autoencoders obtain much better compression efficiency, thanks to higher-capacity encoder/decoder DNN architectures that can be trained on large set of videos (\eg Vimeo-90K~\cite{??}). 
Like traditional codecs, recent video autoencoders compute and compress motion vector estimation and residuals separately, rather than compressing each frame from scratch. 
These optimizations improve not only compression efficiency but also generalization of these NN-based autoencoders.


\mypara{Caveats}
Though various autoencoders are studied extensively in the computer vision community, there has been surprisingly little attention given to careful comparison between autoencoders and traditional codecs (H.265 and H.264), leading to biased (and sometimes exaggerated) perception of autoencoders's performance. 
Traditional video codecs have been extremely heavily engineered, but if one tests an autoencoder and H.265 under the same small (4-10) GoP, autoencoders can outperform H.265, because small GoPs align better with how autoencoders are trained but are not what H.265 is designed for. 
Such comparison can be unfavorable to autoencoders as well.
For instance, H.26x obtains better motion vector estimation and smaller residuals by searching for {\em multiple} reference frames, whereas most designs of autoencoders derive motion vectors and residuals only a {\em single} reference frame (which is not a fundamental constraint), but instead focus on better compression of the motion vectors and residuals.
To make it more complicated, autoencoders are trained to optimize PSNR (pixel distortion) whereas traditional codecs are designed with YUV-SSIM in mind\cite{some citation?}.

With these caveats in mind, we try our best to avoid such pitfalls in our evaluation of autoencoders and their baselines. (For space limitation, we elaborate the details in \S\ref{??}.)
For instance, we evaluate them in both PSNR and YUV-SSIM and do not limit the GoP of H.26x, but use their default encoding setting instead (\eg GoP of \fillme). 
We also disable B-frames (0 bframe and rc-lookahead) and use \texttt{fast} preset in H.26x, as in most real-time videos~\cite{??,??}\footnote{To be clear, we make sure that this is still unfavorable to autoencoders, since H.26x can still use multiple history frames as reference, but autoencoders only use one.}.
\jc{yihua: please find some citation/pointers to justify this choice.}
The bottom line is that our pre-trained autoencoder~\cite{??,??} (which \name customizes) is worse than H.265 with all optimizations, but without b-frame optimization, it is on par with H.265 and better than H.264.


Despite being emergent and relatively less engineered than traditional codecs, autoencoders are increasingly applied by the signal processing community for image compression~\cite{??,??} and wireless communication~\cite{??,??}, by multimedia community for high-volumetric video compression~\cite{??,??} and recently by the networking community to improve chunk-based video streaming~\cite{swift}.
Unlike this work, however, these efforts still rely on packets retransmission or traditional schemes (like FEC) to handle packet losses. 


==> sections/motivate_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Loss tolerance for real-time video}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.92\linewidth]{figs/primitive_table_new.pdf}
    \caption{Abstractions of different loss-resilient schemes. The differences are: 
    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
    (2) unlike retransmission-based or redundancy-based schemes which must retransmit lost packets until some {\em predefined set} or {\em minimum number} of packets are received, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.}
    \label{fig:primitive-table}
\end{figure*}


% Real-time video, it is crucial that enough data is timely received for each frame, so that the high-quality frames can be rendered at a fixed interval (\eg every 50ms for 20fps). 
% However, as most packet networks have occasional congestion, delay jitter and packet losses, not all packets of a frame may arrive timely.
% Retransmitting missing packets is also inefficient if the round trip time is long.
% Therefore, loss-resilient schemes are required to ensure that a frame can be decoded at a high quality even if a fraction of its packets have not arrived when it is supposed to be decoded, \ie non-zero deadline-missing rate or \rate. 



Many recent studies (\eg~\cite{??,??,??,??})\jc{YIHUA, please find more reference} have shown that intermittent congestion, packet jitter, and packet drops are not rare for real-time video applications in the wild. 
Consequently, a client may not have received all packets of a frame when the frame is due for decoding (\eg 40ms after the last frame was decoded if the video is 25fps).

Thus, the ability to tolerate packet losses\footnote{In this work, a packet loss can occur even if the packet is not dropped by the network; a packet is lost if it is delayed (due to congestion, path fluctuation, etc) and arrives after the receiver decodes the frame it belongs to.} is pressingly needed to allow a real-time video client to decode and render the next frame when only a subset of its packets are received.



\subsection{\hspace{-0.3cm}Abstractions of prior loss-resilience schemes}
\label{subsec:abstractions}


%This section revisits three general approaches to loss resilience taken by prior work.  

%\subsection{Prior Loss-Resilient Schemes}

Loss resilience has long been an important research topic. 
While the details vary greatly among different loss-resilient techniques, it helps to view them through the lens of the high-level abstractions that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
These abstractions also influence the interaction with the remaining of a real-time video application, such as congestion control and bitrate adaptation.


\begin{comment}
they have followed some high-level abstractions that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) & \rightarrow \{\texttt{pkts}\}_{sent}\\
%\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}) & \rightarrow \texttt{quality}
%\label{eq:abstraction}
%\vspace{-0.05cm}
%\end{align}
%of certain loss-resilient performance in terms of video quality as a function of received data (packets). 
Viewing them through the lens of abstractions helps us understand their high-level loss-resilience behavior and  with the remaining of a real-time video application, such as congestion control and bitrate adaptation.

\end{comment}

\mypara{Retransmission-based loss resilience}
Packet retransmission is a conventional loss-resilient scheme. 
A client must retransmit packets until a {\em pre-determined set} of packets is reliably delivered. 
Thus the abstraction of retransmission-based loss resilience is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}\subseteq\{\texttt{pkts}\}_{predefined}) &\rightarrow \texttt{quality}\nonumber
\vspace{-0.05cm}
\end{align}
To make it more concrete, we discuss two representative types of retransmission-based schemes.

\smallskip
{\em Single-bitrate coding} must retransmit every lost packet of a video frame for the frame to be decodable. 
When all packets arrive the quality is as high as the original encoded quality.
%This RTX's abstraction can be viewed as ``a frame is non-decodable until all its packets are received, at which point the quality is as high as the original encoded quality.''
This basic scheme is known to have high tail delays if a few packets are resent between two clients whose RTT is higher than inter-frame interval. 

\smallskip
{\em Scalable video coding (SVC)} encodes a video in multiple quality layers, in a way that if a packet of one layer is lost while all packets of lower layers are received, the lower layers can still be decoded.\footnote{\jc{a note on why we dont consider the redundancies in svc}}
Thus, the abstraction of SVC is that ``quality reaches that of the layer $i$ if all packets belonging $i$ and all lower layers have been received.''
That said, a packet loss in SVC can render all higher layers non-decodable. 
For this reason, the base (lowest) layer is often protected by FEC, \ie unequal-protected (UEP) SVC~\cite{wang2000error}, but any packet loss at any other layers can still affect multiple layers. 

Because a pre-determined set of packets will be always be reliably delivered by retransmission, the video coding can focus on compression efficiency (maximal quality under a given target bitrate without any redundancy). 
However, in lack of any redundancy-based techniques, a frame is decodable only if a certain set of packets are received in its entirety, so any lost packets might block the decoding of a frame, making retransmission inevitable in many cases. 
For this reason, most real-time video systems use retransmission together with some redundancy-based loss-resilient techniques, so only a selective set of lost packets need to be resent. 




\mypara{Redundancy-based loss resilience}
Unlike retransmission, redundancy-based techniques trade compression efficiency for loss resilience. 
As long as an enough {\em number} of packets are received, the frame will be decodable at a decent quality. 
The abstraction of redundancy-based loss resilience is characterized by:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, \texttt{redun}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}},\texttt{redun}) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}
This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).
Here, we discuss two concrete redundancy-based schemes.

\smallskip
{\em Forward error correction (FEC)} is widely used in most WebRTC-based real-time video systems.\footnote{\jc{a footnote on the suboptimal use of fec in webrtc}}
Put simply, an idealized FEC takes an encoded video frame (or any file) of size $M$ packets, codes it with redundancy bits, such that the receiver can then recover the data as long as {\em any} $M$ packets\footnote{This work assume equal-sized packets. This is aligned with existing applications, \fillme} are received. 
FEC has been studied intensively in the IEEE multimedia community, with \fillme and \fillme achieving near-ideal performance of FEC and fountain codes. (\cite{??,??} give a more in-depth introduction of FEC.)
Therefore, FEC's abstraction can be described as ``the quality of a frame is low (undecodable) until {\em any} $M$ packets are received.''

FEC suffers the well-known ``cliff effect''. 
For a given data (a frame or chunk encoded by a video coder like H.265), no matter how much redundancy is added, at least as many bytes as in the original data must be delivered, and the decoded video quality remains the same even if more bytes arrive.
Thus, the video encoder should ideally encode each video frame at exact the bitrate that matches the amount of data received when the frame is decoded. 
As a consequence, {\em FEC is effective {\bf if} the sender knows how many bytes can be timely delivered in advance.} 
With less redundancy, the receiver must wait for more packets to arrive or be retransmitted; with more redundancy, the video quality will be low.



\smallskip
{\em Intra-MB insertion}
The multimedia community has also proposed techniques to make video coding (\eg H.264) resilient to packet losses by keep more existing pixel-level redundancy during the video coding process (as opposed to FEC which adds redundancy on top of an encoded frame).
The idea is to reduce the inter-dependencies between macroblocks that are potentially similar to each other. 
For instance, \jc{Yihua, explain R/D optimization, intra-MB insertion, dynamic reference selection, etc}
\jc{need a footnote here to describe how entropy encoding can be stopped at the boundary between packets. }

Like FEC, with more pixel-level redundancy preserved, data erasures have less impact, but compression efficiency is lowered at the same time. 
In practice, with all packets, the decoded quality of intra-MB insertion is lower than that of the coding algorithm that is optimized for coding efficiency (\ie no redundancy), and while a small fraction of data losses can be efficiently tolerated, a high loss rate (more than 40\% data erasure) will still render a frame undecodable~\cite{??,??}. 

\jc{need a footnote to discuss frame skipping and reference frame selection!!!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.85\linewidth]{figs/motivate_example_placeholder.pdf}
         \label{fig:}
    \caption{\jc{YIHUA, let's run WebRTC (with FEC adaptation turned on) on a simple bandwidth trace like this.}}
    \label{fig:motivate-example}
\end{figure}


\mypara{Limitations}
Retransmission-based schemes become less effective than redundancy-based schemes under longer propagation delays between clients. 
However, compared to traditional coders (\eg H.265) that are optimized for video coding efficiency (less bits for higher quality), the redundancy-based abstractions are less efficient in that they use more bits to obtain same quality in the absence of any packet loss.
%That is, they must trade compression efficiency for loss resilience, so the rate of redundancy is highly sensitive to \rate prediction. 
Thus, these abstractions of loss resilience are effective only if they can predict future packet loss rate and jitter, which is not always possible in practice. 

Figure~\ref{fig:motivate-example} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate can adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). 
But this is at the cost of much lower video quality, as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.

\jc{mention the findings corroborate with \cite{\url{https://docs.google.com/document/d/1Hg1SaLEl6T4rEU9j-isovCo8VEjjnuCPTcLNJewj7Nk/edit}}}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.6\linewidth]{figs/motivate_regime.pdf}
    \caption{Traditional abstractions (retransmission-based and redundancy-based) for loss resilience are suitable for connections with low latency or predictable packet loss rates, respectively. However, they are less effective if latency is long and packet loss rate is highly dynamic.}
    \label{fig:motivate-regime}
\end{figure}

To summarize, Figure~\ref{fig:motivate-regime} illustrates when existing schemes are effective.
When the RTT of the connection is low compared to the desirable frame delay, packet retransmission would be sufficient to conceal any packet losses.
When the packet loss rate of the next frame is largely predictable, FEC-based schemes will be sufficient. 
In short, current abstractions fall short in the case of high RTT and highly dynamic packet jitters and losses.



\subsection{Data-scalable video delivery}

To overcome the limitations of prior loss-resilient schemes, we envision a new abstraction of loss resilience---{\em data-scalable} delivery, which entails two specific requirements.
{\em (i)} First, a frame is encoded in a way that is not dependent on the prediction of future packet losses.
%{\em (ii)} Second, the decoded quality with {\em any} $x\%$ ($x>0$) received packets is lower but still comparable to classic codec (\eg H.265) with $x\%$ FEC redundancy.
%Note that classic coder $x\%$ with  can be viewed as a reference design that optimizes compression efficiency, not loss resilience.
{\em (ii)} The frame is decodable once {\em any} non-empty subset of its packets are received and the quality improves with more packets received.
%\item 
%\end{packeditemize}
Using the form of prior loss-resilience abstractions, data-scalable delivery is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}|) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}

Figure~\ref{fig:primitive-table} illustrates the difference between data-scalable delivery and other loss-resilient techniques.
%,  illustrates an example frame whose coded data is delivered in six packets arriving at the receiver at an arbitrary order. 
The most noticeable benefit of data-scalable delivery is that, while the exact arrival time of each packet is unknown to the receiver, data-scalable delivery offers the receiver the {\em flexibility} to decode a frame anytime after receiving any one of the packets. 
Moreover, each new packet strictly improves quality.

It helps to compare data-scalable delivery with SVC whose quality increase with throughput. 
However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets.
As a result, each new packet does not always improve quality until all packets of a higher layer (and all layers below it) have been received. 
In other words, a missing packet may disproportionally render multiple quality layers undecodable. 
For this reason, in practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).




\subsection{Why autoencoder?}
\label{subsec:why-autoencoder}

This work is framework built on autoencoders, an emergent class of learned coders for video frames, including I-frames and P-frames.
Compared to early autoencoder variants, recent autoencoders obtain much better compression efficiency, thanks to higher-capacity encoder/decoder DNN architectures that can be trained on large set of videos (\eg Vimeo-90K~\cite{??}). 
Like traditional codecs, recent video autoencoders compute and compress motion vector estimation and residuals separately, rather than compressing each frame from scratch. 
These optimizations improve not only compression efficiency but also generalization of these NN-based autoencoders.

\mypara{Autoencoder-based data-scalable coding}
We base our approach on autoencoder, not only because of its potential compression efficiency, but more importantly, the performance of several autoencoders (albeit suboptimal) naturally fits the definition of data-scalable delivery. 
For example, we consider a pre-trained I-frame autoencoder~\cite{??} and a pre-trained P-frame autoencoder~\cite{??}. 
To emulate the effect of packet losses, we randomly erase \fillme\% of values in the autoencoder-returned data (without entropy encoding). 
We will explain how this random data erasure simulates packet losses in \S\ref{??}.
Figure~\ref{fig:autoencoder-pretrained} shows that as more data is received, the decoded quality gradually improves. (The test is on a different video dataset than the training dataset.)
It is very encouraging that even the pre-trained autoencoders produce data-scalable delivery.


\begin{figure}[t!]
    \centering
%    \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/psnr-loss-vs-pretrained.pdf}
%         \caption{P-frame model}
%         \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/autoencoder_pretrained_qmap_v1.png}
%         \caption{I-frame model}
%         \label{fig:}
%     \end{subfigure}

         \includegraphics[width=0.6\linewidth]{figs/psnr-loss-vs-pretrained.pdf}

    \caption{Loss resilience of an example pre-trained autoencoder (red). It is already data-scalable (decodable with any subset of packets), but the quality drops much faster than the graceful degradation observed in our solution. \jc{YIHUA, make the figure wider. Swap the order of the legend to "Pre-trained autoencoder" and "Our custom autoencoder"}
%    Our models has a more graceful quality degradation under packet losses comparing to pretrained models
    }
    \label{fig:autoencoder-pretrained}
\end{figure}

However, with these pre-trained autoencoders, the quality grows quite {\em slowly} only a few packets are received. 
This is expected, since these autoencoders are not trained to realize data-scalable delivery. 
Our goal in the remaining of the paper is two-fold: (1) creating better data-scalable autoencoders that produce better quality under various packet losses, and (2) designing a custom real-time video delivery system on top autoencoders as a codec, which strikes better balance between frame delay and video quality. 

\mypara{Caveats of autoencoders}
Though various autoencoders are studied extensively in the computer vision community, there has been surprisingly little attention given to careful comparison between autoencoders and traditional codecs (H.265 and H.264), leading to biased (and sometimes exaggerated) perception of autoencoders's performance. 
Traditional video codecs have been extremely heavily engineered, but if one tests an autoencoder and H.265 under the same small (4-10) GoP, autoencoders can outperform H.265, because small GoPs align better with how autoencoders are trained but are not what H.265 is designed for. 
Such comparison can be unfavorable to autoencoders as well.
For instance, H.26x obtains better motion vector estimation and smaller residuals by searching for {\em multiple} reference frames, whereas most designs of autoencoders derive motion vectors and residuals only a {\em single} reference frame (which is not a fundamental constraint), but instead focus on better compression of the motion vectors and residuals.
To make it more complicated, autoencoders are trained to optimize PSNR (pixel distortion) whereas traditional codecs are designed with YUV-SSIM in mind\cite{some citation?}.

With these caveats in mind, we try our best to avoid such pitfalls in our evaluation of autoencoders and their baselines. (For space limitation, we elaborate the details in \S\ref{??}.)
For instance, we evaluate them in both PSNR and YUV-SSIM and do not limit the GoP of H.26x, but use their default encoding setting instead (\eg GoP of \fillme). 
We also disable B-frames (0 bframe and rc-lookahead) and use \texttt{fast} preset in H.26x, as in most real-time videos~\cite{??,??}\footnote{To be clear, we make sure that this is still unfavorable to autoencoders, since H.26x can still use multiple history frames as reference, but autoencoders only use one.}.
\jc{yihua: please find some citation/pointers to justify this choice.}
Moreover, we always train autoencoders on the same dataset (Vimeo-90K~\cite{??}) but report the test result on different datasets.
The bottom line is that our pre-trained autoencoder~\cite{??,??} (which \name customizes) is worse than H.265 with all optimizations, but without b-frame optimization, it is on par with H.265 and better than H.264.


Despite being emergent and relatively less engineered than traditional codecs, autoencoders are increasingly applied by the signal processing community for image compression~\cite{??,??} and wireless communication~\cite{??,??}, by multimedia community for high-volumetric video compression~\cite{??,??} and recently by the networking community to improve chunk-based video streaming~\cite{swift}.
Unlike this work, however, these efforts still rely on packets retransmission or traditional schemes (like FEC) to handle packet losses. 




% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.99\linewidth]{figs/primitive_example.pdf}
%     \caption{}
%     \label{fig:primitive_example}
% \end{figure}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/primitive_example_new.pdf}
%    \caption{}
%    \label{fig:primitive_example}
%\end{figure*}




%
%
%\jc{need to elaborate on this! need a "functional" description of the data-scalable primitive}
%

\begin{comment}


To  the limitations of the traditional loss-resilient schemes, we choose a different approach, by borrowing the concept of deep autoencoder and exploring its design choices in the context of \name, the first autoencoder-based real-time video system.
% We first describe the design choices of its autoencoder-based codec.

Before delving into the detailed design, we posit two requirements that should be met by an ideal codec for real-time video systems, which we refer to as {\em data-scalable} codec: 
\begin{packeditemize}
\item The video coding should be \rate-agnostic, and 
\item At any \rate ($<100\%$)\footnote{Importantly, the second requirement does {\em not} include \rate of 100\% (no data received).}, the decoded quality is near that of FEC-based loss protection if FEC knows the \rate. 
\end{packeditemize}
For instance, (see Figure~\ref{fig:intro-example}), \name's codec achieves similar quality as H.265 without FEC-based protection
% An example of such codec is the one we developed as part of \name.
As shown in Figure~\ref{??}, when \rate is zero, the quality is similar to that of H.265 without FEC-based protection, and as fewer packets are received (higher \rate) quality degrade {\em gracefully}, achieving similar quality as H.265 protected by an FEC redundancy rate that matches the \rate. 
\end{comment}


% This section introduces the basic design of our data-scalable video codec, and the next few sections will examine its design choices and how it should be used in an end-to-end real-time video system.






==> sections/motivate_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Loss tolerance for real-time video}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.92\linewidth]{figs/primitive_table_new.pdf}
%    \caption{Abstractions of different loss-resilient schemes. The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
%    (2) unlike retransmission-based or redundancy-based schemes which must retransmit lost packets until some {\em predefined set} or {\em minimum number} of packets are received, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.}
%    \label{fig:primitive-table}
%\end{figure*}


% Real-time video, it is crucial that enough data is timely received for each frame, so that the high-quality frames can be rendered at a fixed interval (\eg every 50ms for 20fps). 
% However, as most packet networks have occasional congestion, delay jitter and packet losses, not all packets of a frame may arrive timely.
% Retransmitting missing packets is also inefficient if the round trip time is long.
% Therefore, loss-resilient schemes are required to ensure that a frame can be decoded at a high quality even if a fraction of its packets have not arrived when it is supposed to be decoded, \ie non-zero deadline-missing rate or \rate. 



Many recent studies (\eg~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental}) have shown that intermittent congestion, packet jitter, and packet drops are not rare and can cause long tail delay and low frame rate for real-time video applications. 
Consequently, a client may not have received all packets of a frame when the frame is due for decoding (\eg 40ms after the last frame was decoded if the video is 25fps).
Thus, the ability to decode a frame, despite packet losses (including those dropped or those delayed by congestion), is pressingly needed. 

\begin{comment}
Thus, the ability to tolerate packet losses\footnote{In this work, a packet loss can occur even if the packet is not dropped by the network; a packet is lost if it is delayed (due to congestion, path fluctuation, etc) and arrives after the receiver decodes the frame it belongs to.} is pressingly needed to allow a real-time video client to decode and render the next frame when only a subset of its packets are received.
\end{comment}


\subsection{\hspace{-0.3cm}Abstractions of prior loss-resilience schemes}
\label{subsec:abstractions}


%This section revisits three general approaches to loss resilience taken by prior work.  

%\subsection{Prior Loss-Resilient Schemes}

Loss resilience has long been an important research topic. 
While the details vary greatly among different loss-resilient techniques, it helps to view them through the lens of the high-level abstractions (summarized in Figure~\ref{fig:primitive-table}) that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
These abstractions also influence the interaction with the remaining of a real-time video application, such as congestion control and bitrate adaptation.


\begin{comment}
they have followed some high-level abstractions that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) & \rightarrow \{\texttt{pkts}\}_{sent}\\
%\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}) & \rightarrow \texttt{quality}
%\label{eq:abstraction}
%\vspace{-0.05cm}
%\end{align}
%of certain loss-resilient performance in terms of video quality as a function of received data (packets). 
Viewing them through the lens of abstractions helps us understand their high-level loss-resilience behavior and  with the remaining of a real-time video application, such as congestion control and bitrate adaptation.

\end{comment}

\mypara{Retransmission-based schemes}
%Packet retransmission is a conventional loss-resilient scheme. 
A retransmission-based client takes in a video frame encoded by a traditional codec (\eg H.264) under a target bitrate, and it must resend lost packets until a {\em pre-defined set} of packets (pre-determined before the frame's packets are sent) is reliably delivered. 
This abstraction can be written as:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}\supseteq\{\texttt{pkts}\}_{predefined}) &\rightarrow \texttt{quality}\nonumber
\vspace{-0.05cm}
\end{align}
To make the discussion more concrete, we consider two typical retransmission-based schemes.

\smallskip
{\em Basic TCP-based delivery} must retransmit every lost packet for a frame to be decodable. 
Once all packets are received, the quality will equal the original encoded quality.
%This RTX's abstraction can be viewed as ``a frame is non-decodable until all its packets are received, at which point the quality is as high as the original encoded quality.''
This scheme is known to suffer high tail delays, if the connection has an RTT longer than inter-frame interval.
%if a few packets are resent between two clients whose RTT is higher than inter-frame interval. 

\smallskip
{\em Scalable video coding (SVC)} encodes a video with multiple quality layers, such that a quality layer can be decoded as long as packets of this layer and all lower layers are received.
% \footnote{\jc{a note on why we dont consider the redundancies in svc}}
%if a packet of one layer is lost while all packets of lower layers are received, the lower layers can still be decoded.
%Thus, the abstraction of SVC is that ``quality reaches that of the layer $i$ if all packets belonging $i$ and all lower layers have been received.''
That said, a lost packet can render all higher layers non-decodable. 
Even if the base (lowest) layer is often padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, any packet loss at any other layers can still affect multiple layers. 

The advantage of the retransmission-based approach is that video coding can focus on compression efficiency (maximal quality under a given target bitrate), because a pre-determined set of packets will be always reliably delivered.
However, without any redundancy, a frame is decodable only if a pre-defined set of packets (all packets or those of a few layers) are received in its entirety. 
%any lost packets might block the decoding of a frame, making retransmission inevitable in many cases. 
To avoid blocking the decoding by a missing packet, retransmission is inevitable, but retransmission can be very slow in long-RTT networks, especially when the extra delay to request a lost packet is longer than the jitter buffer (\fillme), which result in a visually perceivable lag or skipped frame.
Therefore, retransmission is also complemented by some redundancy-based loss-resilient techniques, so only fewer lost packets need to be resent. 





\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.995\linewidth]{figs/primitive_table_new_v3.pdf}
    \caption{
Different abstractions of loss-resilient schemes. 
    Retransmission-based schemes (TCP, SVC) obtain high quality (the red horizontal line) but only if a predefined minimum {\em set} of packets are received.
    Redundancy-based ones (FEC, intra-MB) tolerate a pre-defined maximum packet loss rate by adding more redundancy (thus lower quality when all packets are received).
    In contrast, data-scalable delivery can decode a frame from any non-empty set of packets, gradually improves quality with {\em each} new packet, and achieves a high quality when all packets arrive. 
%    The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable delivery does not need to add more redundancy to tolerate more predicted packet losses, and
%    (2) unlike retransmission-based schemes which must receive a predefined minimum {\em set} of packets, data-scalable delivery can decode a frame with any non-empty set of packets.
%    Comparing different abstractions of loss-resilient schemes. The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
%    (2) unlike retransmission-based schemes which must receive a predefined minimum {\em set} of packets, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.
%    (3) unlike redundancy-based ones which must receive a minimum number of packets, data-scalable delivery can decode a frame with 
    }
    \label{fig:primitive-table}
\end{figure}




\mypara{Redundancy-based schemes}
A frame is decodable when at least $N\%$ packets are received, but the decoded quality is lower with a smaller $N$.
Here, $(1-N\%)$ represents the redundancy rate, which depends on the predicted packet loss rate.
Effectively, redundancy-based schemes trade coding efficiency (more bits to obtain same quality) for loss resilience. 
The abstraction is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, N\%) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq N\%,N) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}
%This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).
Redundancy-based schemes have been studied intensively in the IEEE multimedia community~\cite{??,??}.
Two typical redundancy-based schemes are FEC and intra-MB insertion.

%The abstraction of redundancy-based loss resilience is characterized by:
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, \texttt{redun}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
%\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}},\texttt{redun}) &\rightarrow \texttt{quality}\nonumber
%\nonumber
%\vspace{-0.05cm}
%\end{align}
%This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).
%Here, we discuss two concrete redundancy-based schemes.

\smallskip
{\em Forward error correction (FEC)} is widely used in WebRTC-based applications.\footnote{\jc{a footnote on the suboptimal use of fec in webrtc}}. %(see \cite{??,??} for an in-depth discussion).
Ideally, FEC takes an encoded video/frame of size $M$ packets, codes it with redundancy bits, and the receiver can then recover the data if {\em any} $M$ packets\footnote{This work assume equal-sized packets. This is aligned with existing applications, \fillme} are received. 
%, with \fillme and \fillme achieving near-ideal performance of FEC and fountain codes. 
%Therefore, FEC's abstraction can be described as ``the quality of a frame is low (undecodable) until {\em any} $M$ packets are received.''
FEC suffers the well-known ``cliff effect''. 
To send a piece of data,
%(a frame or chunk encoded by a video coder like H.265), 
no matter how much redundancy is added, at least as many bytes as in the original data must be delivered, and the decoded video quality remains the same even if more data are received.
Thus, with less redundancy, the receiver must wait for more packets to arrive or be retransmitted; with more redundancy, the video quality will be low.
%Thus, the video encoder should ideally encode each video frame at exact the bitrate that matches the amount of data received when the frame is decoded. 



\smallskip
{\em Intra-MB insertion} does not explicitly add redundancy like FEC. 
% has also proposed techniques to make video coding (\eg H.264) resilient to packet losses by keep more existing pixel-level redundancy during the video coding process (as opposed to FEC which adds redundancy on top of an encoded frame).
Instead, it reduces the inter-dependencies between macroblocks that are potentially similar to each other. 
For instance, \jc{Yihua, explain R/D optimization, intra-MB insertion, dynamic reference selection, etc}
\jc{need a footnote here to describe how entropy encoding can be stopped at the boundary between packets. }


\jc{need a footnote to discuss frame skipping and reference frame selection!!!}


To tolerate packet losses, both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.
Thus, {\em they are most effective, {\em if} the sender knows how many bytes can be timely delivered in advance}.



\begin{figure}[t!]
    \centering
      \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/webrtc-rate.pdf}
         \caption{Bandwidth and bitrate}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/webrtc-delay.pdf}
         \caption{Frame delay}
         \label{fig:}
     \end{subfigure}
        \label{fig:}
    \caption{\jc{YIHUA, let's run WebRTC (with FEC adaptation turned on) on a simple bandwidth trace like this.}}
    \label{fig:motivate-example}
\end{figure}


Unfortunately, predicting how many packets will not arrive by time is hard. 
Figure~\ref{fig:motivate-example} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate can adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). 
But this is at the cost of much lower video quality, as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.

\jc{mention the findings corroborate with \cite{\url{https://docs.google.com/document/d/1Hg1SaLEl6T4rEU9j-isovCo8VEjjnuCPTcLNJewj7Nk/edit}}}

\jc{also mention that fec is not native in webrtc. this is google implementation}

%Like FEC, with more pixel-level redundancy preserved, data erasures have less impact, but compression efficiency is lowered at the same time. 
%In practice, with all packets, the decoded quality of intra-MB insertion is lower than that of the coding algorithm that is optimized for coding efficiency (\ie no redundancy), and while a small fraction of data losses can be efficiently tolerated, a high loss rate (more than 40\% data erasure) will still render a frame undecodable~\cite{??,??}. 


\begin{comment}

\mypara{Limitations}
Retransmission-based schemes become less effective than redundancy-based schemes under longer propagation delays between clients. 
However, compared to traditional coders (\eg H.265) that are optimized for video coding efficiency (less bits for higher quality), the redundancy-based abstractions are less efficient in that they use more bits to obtain same quality in the absence of any packet loss.
%That is, they must trade compression efficiency for loss resilience, so the rate of redundancy is highly sensitive to \rate prediction. 
Thus, these abstractions of loss resilience are effective only if they can predict future packet loss rate and jitter, which is not always possible in practice. 

Figure~\ref{fig:motivate-example} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate can adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). 
But this is at the cost of much lower video quality, as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.6\linewidth]{figs/motivate_regime.pdf}
    \caption{Traditional abstractions (retransmission-based and redundancy-based) for loss resilience are suitable for connections with low latency or predictable packet loss rates, respectively. However, they are less effective if latency is long and packet loss rate is highly dynamic.}
    \label{fig:motivate-regime}
\end{figure}

\end{comment}


%Figure~\ref{fig:motivate-regime} illustrates when existing schemes are effective.
In short, retransmission-based schemes are sufficient if the RTT between the clients is low enough to conceal the retransmission delay. 
%compared to the desirable frame delay, packet retransmission would be sufficient to conceal any packet losses.
Redundancy-based schemes are suitable to connections with largely predictable packet loss rate.
% of the next frame is largely predictable, FEC-based schemes will be sufficient. 
However, both of them fall short under high RTT and highly dynamic packet jitters and losses.



\subsection{New abstraction: Data-scalable delivery}

To overcome the limitations of prior loss-resilient schemes, we envision a new abstraction of loss resilience---{\em data-scalable} delivery, which entails two specific requirements.
{\em (i)} First, the frame is decodable once {\em any} non-empty subset of its packets are received, and quality improves with more packets received (or equivalently, quality degrades gracefully with more packets missing).
{\em (ii)} Second, unlike the redundancy-based approach, how a frame is encoded should not depend on the prediction of future packet losses.
%{\em (ii)} Second, the decoded quality with {\em any} $x\%$ ($x>0$) received packets is lower but still comparable to classic codec (\eg H.265) with $x\%$ FEC redundancy.
%Note that classic coder $x\%$ with  can be viewed as a reference design that optimizes compression efficiency, not loss resilience.
%\item 
%\end{packeditemize}
Using the form of prior loss-resilience abstractions, data-scalable delivery is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}|) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}

Figure~\ref{fig:primitive-table} illustrates the difference between data-scalable delivery and other loss-resilient techniques.
%,  illustrates an example frame whose coded data is delivered in six packets arriving at the receiver at an arbitrary order. 
The most noticeable benefit of data-scalable delivery is that, while the exact arrival time of each packet is unknown to the receiver, data-scalable delivery offers the receiver the {\em flexibility} to decode a frame anytime after receiving any one of the packets. 
Moreover, each new packet strictly improves quality.

It helps to highlight the difference between data-scalable delivery and SVC whose quality also increases with more packets. 
However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets.
As we will show in \S\ref{sec:eval}, SVC (even with FEC-protection on the base layer as commonly used~\cite{??,??}) does not always improve quality with each new packet, until all packets of a higher layer (and all layers below it) have been received. 
In other words, a missing packet may render multiple quality layers undecodable. 
%For this reason, in practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).




\subsection{Why autoencoder?}
\label{subsec:why-autoencoder}

Our work is built on autoencoders, an emergent class of neural network coders for video frames, including I-frames and P-frames.
The recent autoencoders borrow ideas from traditional codecs (\eg compressing motion vectors and residuals separately, rather than compressing each frame from scratch), but replace handcrafted heuristics with multi-layer neural nets (NNs) which are trained on large sets of videos (\eg Vimeo-90K~\cite{??}). 
Thanks to these trends, their compression efficiency and generalization have been improving over the recent years.

%Recent autoencoders have improved their compression efficiency, thanks to higher-capacity encoder/decoder DNN architectures, which can be trained on large set of videos (\eg Vimeo-90K~\cite{??}). 
%
%%Like traditional codecs, recent video autoencoders compute and compress motion vector estimation and residuals separately, rather than compressing each frame from scratch. 
%These optimizations improve not only compression efficiency but also generalization of these NN-based autoencoders.

\mypara{Autoencoder-based data-scalable coding}
We base our approach on autoencoders, not because of their compression efficiency, but because their performance (albeit suboptimal) potentially fits the definition of data-scalable delivery. 
For example, we consider a pre-trained P-frame autoencoder~\cite{dvc}. 
To emulate the effect of different packet loss rates, we randomly zero \fillme-\fillme\% of values in the autoencoder-returned data (before entropy encoding). 
(We will explain how such random data erasure simulates packet losses in \S\ref{??}.)
Figure~\ref{fig:autoencoder-pretrained} (red curve) shows that as more data is received, the decoded quality gradually improves. 
(To avoid overfitting, we test it on a different video dataset than the training dataset.)
%It is very encouraging that even a pre-trained autoencoder leads to a (suboptimal) data-scalable delivery.


\begin{figure}[t!]
    \centering
%    \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/psnr-loss-vs-pretrained.pdf}
%         \caption{P-frame model}
%         \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/autoencoder_pretrained_qmap_v1.png}
%         \caption{I-frame model}
%         \label{fig:}
%     \end{subfigure}

         \includegraphics[width=0.6\linewidth]{figs/psnr-loss-vs-pretrained.pdf}

    \caption{Loss resilience of an example pre-trained autoencoder (red). It is already data-scalable (decodable with any subset of packets), but the quality drops much faster than the graceful degradation observed in our solution. \jc{YIHUA, make the figure wider. Swap the order of the legend to "Pre-trained autoencoder" and "Our custom autoencoder"} \jc{also add a horizontal line of H.264/265 without loss}
%    Our models has a more graceful quality degradation under packet losses comparing to pretrained models
    }
    \label{fig:autoencoder-pretrained}
\end{figure}

However, the quality of the pre-trained autoencoder grows quite {\em slowly} when only a few packets are received. 
This is expected, since these autoencoders are not trained to realize data-scalable delivery. 
Our goal in the remaining of the paper is two-fold: (1) creating better data-scalable autoencoders that produce better quality under various packet losses (see the blue line in Figure~\ref{fig:autoencoder-pretrained}), and (2) designing a custom real-time video delivery system that uses autoencoders as a codec, to better balance between frame delay and video quality. 

Despite being emergent and relatively less engineered than traditional codecs, autoencoders are increasingly applied by the signal processing community for image compression~\cite{??,??} and wireless communication~\cite{??,??}, by multimedia community for high-volumetric video compression~\cite{??,??} and recently by the networking community to improve chunk-based video streaming~\cite{swift}.
Unlike this work, however, these efforts still rely on packets retransmission or traditional schemes (like FEC) to handle packet losses. 


\subsection{Caveats of using autoencoders}

Though autoencoders are studied extensively in the computer vision community, there has been surprisingly little attention given to a thorough comparison between autoencoders and traditional codecs (H.265 and H.264), which have been extremely heavily engineered in the multimedia community.
We are aware of that this leads to potentially biased (and sometimes exaggerated) perception of autoencoders's performance. 
%Traditional video codecs have been extremely heavily engineered, but 
For instance, if one tests an autoencoder and H.265 under the same small (4-10) GoP, autoencoders will outperform H.265, because small GoPs align better with how autoencoders are trained but are not what H.265 is designed for. 
On the other hand, a comparison can be unfavorable to autoencoders as well.
For instance, H.26x obtains better motion vector estimation and smaller residuals by using {\em multiple} reference frames, whereas most autoencoders derive motion vectors and residuals only a {\em single} reference frame (which is not a fundamental constraint) and instead focus on better compression of the motion vectors and residuals.
To make it more complicated, autoencoders can optimize either PSNR or SSIM (in RGB or YUV), so research on autoencoders typically evaluate only the metric that the model is trained on.
%whereas traditional codecs are designed with YUV-SSIM in mind\cite{some citation?}.

In this project, we have spent great effort to improvement the performance of autoencoder-based real-time videos (some key optimizations are explained in \S\ref{subsec:optimize}).
We have also tried our best to avoid such pitfalls in our evaluation of autoencoders and their baselines. (For space limitation, we elaborate the details in \S\ref{??}.)
For instance, we evaluate them in various metrics (PSNR and SSIM) and use H.26x's default encoding setting without limiting GoP, and stress-test autoencoders on video sets different from the training set.
We also disable B-frames (0 bframe and rc-lookahead) and use \texttt{fast} preset in H.26x, as in most real-time videos~\cite{??,??}.
\jc{yihua: please find some citation/pointers to justify this choice.}
%train autoencoders on the same dataset (Vimeo-90K~\cite{??}) but report the test result on different datasets.
%Moreover, we allow H.26x can still use multiple history frames as reference, but only one frame as reference in autoencoders. 
%To be clear, we make sure that this is still unfavorable to autoencoders, since H.26x can still use multiple history frames as reference, but autoencoders only use one.
The bottom line is that in our testing, our pre-trained autoencoder~\cite{??,??} (which \name customizes) it is on par with H.265 and better than H.264, and we have also confirmed that in the most aggressive encoding mode (\eg with B-frames and \texttt{fast}), H.265 achieves higher compression efficiency than autoencoders. 

We hope to present a balanced view in this work: even though the autoencoders have lower coding efficiency than the heavily engineered video codecs like H.265, we believe that their potential to reduce tail delay (via data-scalable delivery) outweighs the slightly lowered quality, which is also being constantly improved by better neural-network models.




% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.99\linewidth]{figs/primitive_example.pdf}
%     \caption{}
%     \label{fig:primitive_example}
% \end{figure}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/primitive_example_new.pdf}
%    \caption{}
%    \label{fig:primitive_example}
%\end{figure*}




%
%
%\jc{need to elaborate on this! need a "functional" description of the data-scalable primitive}
%

\begin{comment}


To  the limitations of the traditional loss-resilient schemes, we choose a different approach, by borrowing the concept of deep autoencoder and exploring its design choices in the context of \name, the first autoencoder-based real-time video system.
% We first describe the design choices of its autoencoder-based codec.

Before delving into the detailed design, we posit two requirements that should be met by an ideal codec for real-time video systems, which we refer to as {\em data-scalable} codec: 
\begin{packeditemize}
\item The video coding should be \rate-agnostic, and 
\item At any \rate ($<100\%$)\footnote{Importantly, the second requirement does {\em not} include \rate of 100\% (no data received).}, the decoded quality is near that of FEC-based loss protection if FEC knows the \rate. 
\end{packeditemize}
For instance, (see Figure~\ref{fig:intro-example}), \name's codec achieves similar quality as H.265 without FEC-based protection
% An example of such codec is the one we developed as part of \name.
As shown in Figure~\ref{??}, when \rate is zero, the quality is similar to that of H.265 without FEC-based protection, and as fewer packets are received (higher \rate) quality degrade {\em gracefully}, achieving similar quality as H.265 protected by an FEC redundancy rate that matches the \rate. 
\end{comment}


% This section introduces the basic design of our data-scalable video codec, and the next few sections will examine its design choices and how it should be used in an end-to-end real-time video system.






==> sections/motivation.tex <==
\tightsection{Motivation}

\tightsubsection{Architecture of real-time video conferencing systems}

Propose a model to describe the system. (Video -> encoding algorithm -> packets -> lossy network -> packets' -> decoding algorithm -> reconstructed video)

\tightsubsection{Impact of packet losses}

Some measurements and experiments to show that
\begin{itemize}
    \item packet loss is unavoidable and unpredictable
    \item current hand-crafted methods cannot perform well: RTX-based method cause huge delay. Loss recovery mechanisms may have big quality degradation under some scenarios.
\end{itemize}

\tightsubsection{Goal of our design}
Have a graceful quality without retransmission under packet losses.

==> sections/overview.tex <==
\tightsection{Autoencoder: A learning-based solution}
To achieve the goals proposed above, we consider the autoencoder, a learning based approach for codecs. In this sections, we ...

\tightsubsection{What to learn}
\begin{itemize}
    \item An autoencoder which still delivers decent quality under packet losses
\end{itemize}

\tightsubsection{Why learning}

\begin{itemize}
    \item During training, autoencoder can see various loss patterns from the data. Therefore, it has a better potential to deal with varying loss rates.
    \item Autoencoders can automatically learn which part of data is more critical to the quality in an end-to-end manner. 
    \item ...
\end{itemize}

\tightsubsection{How to learn}
Present an overview of our training process -- how to train with loss.

==> sections/related_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Related Work}
\label{sec:related}

% \begin{itemize}
% \item loss resilient schemes
% \item adaptive streaming: cc, fec rate, bitrate, etc.
% \item autoencoders
% \end{itemize}

% Other than the prior work elaborated elsewhere, we want to briefly mention a few other related techniques.


\mypara{Adaptive video streaming}
Loss-resilient video coding can be codec-specific (\eg~\cite{rdo,salsify} discussed in \S\ref{sec:motivate}) or adapt
% As the codecs become standardized and widely used in popular platforms like WebRTC, recent efforts shift focus to adapting 
common configurations of codecs or error correction (\eg FEC)~\cite{holmer2013handling}.
There has been intense research on adaptive video streaming, including performance analysis of commercial players (\eg~\cite{macmillan2021measuring,carlucci2016analysis}) and how to better adapt packet retransmission (\eg~\cite{feamster2002packet,yang2005unequal}), sending rate (\eg~\cite{sprout,concerto}), encoding bitrate (\eg~\cite{salsify,xiao2018two,zhang2021loki}) and FEC redundancy rate (\eg~\cite{nagy2014congestion,fong2019low}), which seek to predict future network conditions and/or quickly react to any changes. 
However, these predictions are not always accurate. %, due to occasional packet losses/delaying. 
% as the tail delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
% While they achieve good performance with accurate predictions, it not easy to always be accurate, and thus the tail quality and delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
In contrast, data-scalable coding is complementary to rate adaptation, but they eschew the need for accurate loss prediction and instead gracefully degrade their quality with more packet losses.

\begin{comment}

\mypara{Loss-resilient video coding}
Most early work on loss-resilient video coding focuses on modifying traditional codec (\eg H.26x) so that the decoder can reconstruct frames at decent quality in lossy networks (see FEC~\cite{holmer2013handling}, RDO~\cite{rdo}, and stateful encoding~\cite{salsify} for specific examples in \S\ref{sec:motivate}).
As the codecs become standardized and widely deployed in devices, recent efforts shift focus to adapting configurations (\eg reference frames, target bitrate) of these codecs and block error correction (FEC) to enhance loss resilience~\cite{holmer2013handling}.
% For instance, FEC is supported in WebRTC and other commercial video players~\cite{holmer2013handling}.

As elaborated in \S\ref{sec:motivate}, to obtain robustness to potential packet losses, these techniques must sacrifice encoded quality under no losses.
While \name trades quality for resilience, the tradeoffs are much more favorable, as the compression and loss resilience are jointly optimized.

\mypara{Adaptive video streaming}
There has been intense research on adaptive video streaming, including detailed performance measurements of commercial players (\eg~\cite{macmillan2021measuring,carlucci2016analysis}) and how to better adapt packet retransmission (\eg~\cite{feamster2002packet,yang2005unequal}), sending rate (\eg~\cite{sprout,concerto}), encoding bitrate (\eg~\cite{salsify,xiao2018two}) and FEC redundancy rate (\eg~\cite{nagy2014congestion,fong2019low}) to predict the future network conditions and quickly react to any changes. 
However, these predictions may not be always accurate, as the tail quality and delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
% While they achieve good performance with accurate predictions, it not easy to always be accurate, and thus the tail quality and delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
In contrast, \name eschews the need for accurate loss prediction and instead gracefully degrades its quality with more packet losses.
% since packet losses have a relatively mild impact on video quality and frame delay.

\end{comment}

\mypara{Autoencoder in signal processing}
% Like many deep-learning techniques, applications of neural autoencoders is an active  topic. %~\cite{??,??,??}.
Our work is related to two autoencoder applications in the signal processing community. % are most relevant to this work.
One improves lossy channel communication by training the decoder as a classifier~\cite{erpek2020deep,dai2020deep}. 
To send a message from a set of $n$ messages, the sender encodes a one-hot vector (with the index of the message set to one), and the decoder classifies (possibly corrupted) data to predict which message it is. 
The other uses autoencoders to code images in a representation that is both compact and robust to signal noises~\cite{bourtsoulatze2019deep,gunduz2019machine}.
Like us, it combines data (image) compression with robustness to low SNR in the physical layer. 

Our work differs on two key fronts. 
The first is that they target a different network layer.
Physical-layer protection against signal noises is different from (and complementary to) transport-/application-layer protection against packet losses.
%Physical-layer noises affected data transmission differently than drops/queuing of data packets on which modern real-time video applications (\eg WebRTC) operate. 
Moreover, though physical-layer noises can be modeled as differentiable linear transformations (as in~\cite{bourtsoulatze2019deep,gunduz2019machine}), packet drops (\rate) are not differentiable and need to be handled differently (see \S\ref{sec:design}). 
The second is compressing and streaming videos is different from (if not more difficult than) compressing individual images. 
Video frames cannot be treated separately, because any error on one frame may propagate to future frames. 
While more research is needed, we believe that we have taken a significant step forward in showing the promise of autoencoders in real-time videos and outlining the concrete technical steps that should be pursued. 

\jc{add more on fountain coding}


\section{Limitations}

\mypara{At least one packet has to arrive}
\name cannot decode a frame with no received packet, rather it allows the receiver to choose when to decode {\em after} the first packet arrives. 
This means \name will not help during network disconnection or severe congestion that block any packet arrivals.
One potential way to avoid such extreme situation is leverage multiple concurrent connections and run \name over multipath TCP (with custom packet scheduling to discard or deprioritize untimely packets.)


\mypara{Bounded by autoencoder's performance}
Though \S\ref{sec:eval} shows that \newae's compression efficiency is comparable to H.264 under no packet loss, its quality-bitrate tradeoff is bounded by that of the pre-trained autoencoders. 
This is expected, since we choose not to modify the autoencoder architecture, and instead only train them to be data-scalable. 
Similarly, \newae does not improve the generalization of pre-trained autoencoders on unseen videos, because we train them using the pre-trained models' training data (Vimeo-90K and \fillme).
That said, autoencoders are being constantly improved to obtain higher compression efficiency (\eg via using more reference frames like in traditional codecs) and work better on new videos (\eg via model adaptation).

\mypara{No multi-party support (yet)}


\mypara{First I-frame must be lossless}

\mypara{Frames are rarely skipped}


\mypara{Compute and power overhead}





==> sections/technical.tex <==
\tightsection{\name: a loss-resilient autoencoder}
In this section, we describe the design and implementation of our system.

\begin{itemize}
\item 4.1 Basic design of a loss-resilient autoencoder
\begin{itemize}
    \item architecture: i-frame, p-frames, etc
    \item (the difference might be here)
    \item training process: emulate losses and quantization, and what's the loss function
    \item inference process: how to apply entropy encoding (at the per-packet level). only basic design here, we will cover rate adaptation later
    \item how is it different from other autoencoders? (architecture, training, inference)
\end{itemize}
\item 4.2 Understanding the design choices
\begin{itemize}
    \item show a few examples of "graceful degradation" vs. training loss rate
    \item how to set the loss rate in training?
\end{itemize}
\item 5. practical issues
\begin{itemize}
    \item 5.1 bitrate adaptation (qp for rate adaptation)
    \item 5.2 adapting coding overhead (resizing for compute/delay budget)
    \item 5.3 streaming protocol for reference frame synchronization
    \item 5.4 
\end{itemize}
\item 6. Implementation
this could be folded to 5.4 if not too much to say
\begin{itemize}
    \item putting it together in webrtc: interface with webrtc (including rate adaptation, compute adaptation, frame-sync protocol). 
    \item implementation optimization
\end{itemize}
\end{itemize}


\tightsubsection{Basic design of \name}
Figure~\ref{?} presents a high-level overview of \name. It consists of three main components: an I-frame encoder/decoder, a P-frame encoder/decoder, and an entropy coder. 
For the I-frame encoder/decoder, we leverage the design proposed by Song \etal\cite{QMAP}. Figure~\ref{?} presents its workflow. The I-frame encoder takes a single image as the input and outputs a latent vector as the encoded frame. The latent vector will then be compressed into packets via lossless entropy coding (will introduce shortly) and sent out to the network. On the receiver side, it will first perform entropy decoding to restore the latent vector, which will then be fed into the decoder neural network to reconstruct the image.

To encode/decode the P-frames, we use the design from Lu \etal\cite{DVC} as shown in Figure~\ref{?}. The input to the P-frame encoder includes two parts: (i) the image to be encoded, and (ii) the reference image. The output latent vector of the P-frame encoder will also be compressed via entropy encoding and decompressed at the receiver side. The P-frame decoder takes the received latent vector as well as the reference frame as the input and outputs the reconstructed image
%We note that unlike H.264 which uses the previous image as the reference\cite{?}, the reference image selection for the our P-frame encoder/decoder is much more flexible. It can be any image comes before the current one.

\yh{TODO: describe the entropy coding component}
\yh{TODO: describe the differences of our design compared with Qmap and DVC}

\mypara{Training strategy} To make our codec loss resilient, we retrain both the I-frame codec and the P-frame codec with emulated packet losses. More specifically, \yh{describe how we add loss and why that is differentiable (every byte in the latent vector has \fillme\% of the chance to be zeroed-out)}. We use ADAM optimizer to retrain the I-frame codec and the P-frame codec for \fillme and \fillme iterations respectively on an Nvidia 3080 GPU. We train the I-frame codec using the \fillme dataset and the P-frame codec is trained on the Vimeo-90K dataset\cite{xue2019video}. All the training images are cropped into 256x256 pieces to fit the GPU memory. We adopt the loss function and the quantization method from the previous works \cite{DVC, QMAP}.

\mypara{Inference strategy} In \name, we use entropy coding to provide lossless compression for the latent vector. Usually, a P-frame with 720P resolution will be compressed into \fillme packets. However, the loss of a single packet can break the entropy coding and make the compressed latent vector unrecoverable on the receiver side. To address this problem, we apply a per-packet entropy coding mechanism. That is, we partition the latent vector into multiple chunks and apply entropy coding for each chunk independently. We adjust the size of each chunk based on the number of bytes after entropy coding so that they can fit into one packet. Per-packet entropy coding may incur an overhead when compared with one-time entropy coding. However, as we will show in section \fillme, such overhead is negligible.

Besides entropy coding, packet loss can still cause another problem: loss of one packet will zero out a large consecutive area in the latent vector, which may make the decoder hard to reconstruct the original image in practice. To address this problem, we apply a reordering algorithm to the latent vector before entropy coding. \yh{describe this algorithm in a mathematical way.}  After reordering, the packet loss will zero out multiple small chunks spread uniformly across the whole latent vector. The experiment result (in section \fillme) shows that adding the reordering algorithm can improve {\fillme}db in PSNR when comparing to the default pipeline without reordering.

To cooperate with the congestion control component in video conferencing applications, \name also provides an interface for bitrate adaptation during inference. It takes a value, $Q$, between 0 and 1 as the input and adjust the quality-size trade-off. When $Q = 0$, \name will encode the frame with the lowest quality and thus with the smallest size. When $Q=1$, \name will encode the frame with highest quality and largest size. We will introduce the detailed bitrate adaptation mechanism in section \fillme.

%Although the model trained with loss can handle information loss in the latent vector during training, packet loss can 
%Besides the lost of information, packet losses during inference can cause two extra problems: \emph{(i)} packet losses will break the entropy coding, and \emph{(ii)} data loss of consecutive-area in latent vector is hard to recover. 

 
\begin{figure}[t!]
    \centering
         \centering
         \includegraphics[width=0.75\linewidth]{figs/design-choice-placeholder.png}
         \label{fig:}
    \caption{(placeholder) Autoencoders can tolerate a much larger loss rate during inference when training with a relatively smaller loss rate. \yh{adding a line/subgraph showing if loss during training is too high, performance will be bad} \yh{add Qmap}}
    \label{fig:design-choice-profiling}
\end{figure} 

\tightsubsection{Design choices in \name}
As we discussed above, training with loss can help the model become loss resilient. However, there are still two unanswered question: 
\begin{packeditemize}
    \item How much improvement in image quality does the model trained with loss have, comparing to the model trained without loss.
    \item How much loss rate we should use during training?
\end{packeditemize}

Figure~\ref{fig:design-choice-profiling} shows the image quality measured in PSNR under different loss rate during inference. The key insight is: models trained with a low loss rate (such as 20\% and 30\%) is good enough to handle a much higher loss rate (such as 50\% and 60\%) during inference. For I-frame codec, \yh{add experiment for Qmap}.  For P-frame codecs, when we apply 60\% loss during inference, the PSNR of decoded image is \review{35}db when using a model trained with 30\% loss, while the model trainied without loss only provide a image of \review{28.5}db PSNR.

Therefore, we choose \fillme\% and \review{30}\% of loss for training the I-frame codec and the P-frame codec respectively. 

\tightsection{Practical issues}
\yh{think about a better name!}

\tightsubsection{Adapting to varying bitrates}

\tightsubsection{Adapting for coding overhead}

\tightsubsection{Synchronizing reference frames between encoder and decoder}

\tightsection{Implementation}

\begin{comment}
\tightsubsection{Handling packet losses with \name}
\begin{itemize}
    \item In practice, packet loss will bring multiple challenges to the codec
    \begin{itemize}
        \item packet loss will break the entropy coding
        \item Lost of consecutive-area in latent vector is hard to recover
        \item Error caused by packet losses may propagate along P-frames and cause persistent quality degradations
    \end{itemize}
    \item To address those challenges, we propose the following mechanisms: per-packet entropy coding, reorder the latent vector, and explicit synchronization of reference frame between encoder and decoder  
\end{itemize}

\tightsubsection{Bitrate adaptation}
\begin{itemize}
    \item In a video conferencing system, the codec should be able to cooperate with underlying congestion-control system by adjusting its output bitrate.
    \item Our bitrate adaptation mechanism is similar to Salsify (can encode multiple times to choose a suitable encoding parameter)
    \item Encode a single frame for multiple times may incur performance issues. We apply XXX optimization. As we shown in evaluation xxx, \name can provide a decent encoding speed while doing a good adaption to varying target bitrates. 
\end{itemize}

\tightsubsection{Implementation}
How autoencoder is integrated into ffmpeg
\end{comment}

==> sections/technical_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\newcommand{\Coder}{\ensuremath{C_\phi}\xspace}
\newcommand{\Decoder}{\ensuremath{D_\theta}\xspace}
\newcommand{\Quality}{\ensuremath{F}\xspace}
\newcommand{\Packetize}{\ensuremath{A}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\x}{\ensuremath{\textbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\textbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\textbf{z}}\xspace}
\newcommand{\loss}{\ensuremath{p_{\textrm{loss}}}\xspace}




\section{\newae: Data-Scalable Autoencoder}

\name is a concrete instantiation of data-scalable delivery. 
At a high level, \name entails a new autoencoder, \newae, and a custom delivery framework that leverages the properties of \newae.
We will describe \newae in this section, followed by the delivery framework in the next section. 

We begin with the basic terminology of autoencoders. 
We denote the coder (a neural network parameterized by weights $\phi$) by $\Coder$ and the decoder (a neural network parameterized by weights $\theta$) by $\Decoder$.
For an input frame $\x$ in the space of $\X$, the coded data $\z=\Coder(\x)$ will be sent to the receiver, which then decodes $\z$ to reconstruct the original frame $\hat{\x}=\Decoder(\z)$.
Note that the coder and decoder functions do not include the lossless entropy coding and FEC coding; instead, they perform the lossy compression, like the block-based motion estimation and residual computation. 


The compression efficiency of the output $\hat{\x}$ is measured a function $\Quality(\hat{\x},\x)$ by a weighted sum of its visual quality (\eg PSNR) and its entropy-coded size (\eg estimated by a pre-trained neural net), with the weight of visual quality being $\alpha$. 
With a higher value of $\alpha$, the trained $\Coder(\x)$ will produce output $\z$ that naturally leads to better visual quality in $\Decoder(\z)$ but higher file size. 
To adapt to the dynamic sending rate, we train multiple versions of the autoencoders with different weight $\alpha$. (See \name's bitrate adaptation in \S\ref{??}.) 
% A higher $\Quality$ value is better (higher visual quality and/or lower entropy-coded size).


\subsection{Basic formulation of \newae training}

Unlike existing applications of autoencoders, we want to train a {\em data-scalable autoencoder} that not only improves compression efficiency but also is resilient to packet losses.
To this end, we make a few critical changes to the training process of autoencoders.
We customize two existing autoencoder architectures, \cite{dvc} for P-frames (with motion vectors and residuals as input) and \cite{qmap} for I-frames (with a static image as input).\footnote{We do not consider B-frames are they are not commonly used in low-latency videos.} 
We borrow their neural network architectures (their architectures in details in \jc{need an appendix on how dvc creates input \x from two frames, and which part of it was trained by us, which part are not.}).
Since they share the same conceptual framework described above, we do not discuss them separately unless necessary.

The fact that $\Coder$, $\Decoder$, and $\Quality$ are differentiable allows end-to-end training of the autoencoder architecture~\cite{??,??,??}.
Mathematically, given a training set $\X$, our goal is 
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\z = \Coder(\x)
\label{eq:1}
\vspace{-0.05cm}
\end{align}


This traditional training process (Eq.~\ref{eq:1}) can be viewed as having zero \rate, \ie the input to the decoder is the same as the output of the encoder. 
To incorporate non-zero \rate, \name proposes a custom training process for autoencoders, by adding a random distribution $\loss$:
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\highlight{blue}{$\z\sim \loss(\z | \Coder(\x))$}
\label{eq:2}
\vspace{-0.05cm}
\end{align}

We highlight the change in color. 
Based on coder output $\Coder(\x)$, $\loss$ returns a distribution over the possible received data seen by the decoder (after packet erasures under non-zero \rate). 
This randomization effectively lets the training process see the effect of non-zero \rate. 




% \section{Simulating \rates in autoencoder training}



% \mypara{How to simulate packet losses}

\mypara{Key issues of simulating \rates in autoencoder training}
Training a data-scalable autoencoder using Eq.~\ref{eq:2} entails three key questions:
\begin{packedenumerate}
\item How to make Eq.~\ref{eq:2} differentiable for a wide range of $\loss$ that simulates various packet loss patterns?
\item How to convert $\Coder(\x)$ to data packets? This decides how losing a packet would affect the data seen by the decoder.
\item What \rates should be simulated in training, so that the trained model can deal with a range of unseen \rates?
\end{packedenumerate}
% The first question concerns packetization of the coder output and the second question concerns what \rates should be used to train the model that can deal with a range of \rates.
These questions are not involved in canonical autoencoder training, but they become critical here for the need to simulate packet losses in the training process.
% , so that the trained model can handle packet losses of various \rates in real networks. 

\subsection{How to make \newae trainable?}

An immediate challenge imposed by Eq.~\ref{eq:2} is how to train an autoencoder (the weights in $\theta$ and $\phi$), despite that the random distribution $\loss$ is not a naturally differentiable step. 

% that the expected value of $\Quality$ may not always be written in a closed, differentiable form, so before we discuss how \loss simulate packet losses with a non-zero \rate, we must first be able to run backpropagation for weights $\theta$ and $\phi$ in Eq.~\ref{eq:2}. 


\jc{Yihua/Anton, please explain how you used REINFORCE trick here.
\begin{itemize}
    \item this may look like VAE, so a natural solution is reparameterization. it doesn't work because the expectation of $\Quality$ cannot be writtein in a closed, differentiable form
    \item we use reinforce trick.. how does it work?
\end{itemize}}


\subsection{How to simulate packet losses in training?}

\jc{start with how WE do packetization, including per-packet entropy coding, and then list the alternatives}

\jc{an illustration figure here}

As illustrated in Figure~\ref{??} packetization of \name first uses an assignment function $\Packetize$ to map each element of $\z=\Coder(\x)$ to $k$ non-overlapping sublists, and then losslessly encodes each sublist to get the bit stream of a packet.
Conversely, depacketization of \name first losslessly decodes each packet to a sublist and maps the sublists back to $\z$ by the inverse function $\Packetize^{-1}$.
Each packet is numbered so if a packet has not arrived when decoding, the elements mapped it will be set to zero (this is a natural choice, though we will discuss alternatives in \S\ref{??}). 

The key to a good packetization lies in the assignment function $\Packetize$, because it decides how missing one packet would affect the coded data seen by the receiver. 
The lossless coding can use any off-the-shelf entropy coder, and the entropy-encoded bit stream should fit in the size of a packet (1.5KB).
We will discuss our choice of the entropy coder in more details in \S\ref{??}.

We consider three design choices for $\Packetize$:
\begin{packeditemize}
\item Block-based assignment splits $\z$ to {\em contiguous} blocks so elements close together will be encoded in the same packet, much the same way video data is packetized today. 
This serves a reference design point.
\item Interleaving assignment assigns the $i^{\textrm{th}}$ element to the $(i\textrm{ mod }k)^{\textrm{th}}$ packet, where $k$ is the number of packets.
Interleaving-based packetization is recommended by some traditional loss-resilient schemes~\cite{??}.
\item Randomized assignment uses a pseudo-random mapping $\Packetize_{random}$ to assign each element in $\z$ to its position in a packet. 
An inverse function $\Packetize_{random}^{-1}$ (\eg\fillme) can then be used to map the packet data back to $\z$). 
\end{packeditemize}
Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (based on \rates selected in \S\ref{??}). 


\myparaq{Why randomized assignment}
\name chooses randomized assignment over the block-based and the interleaving ones. 
The intuitive reason is that 

\jc{\begin{itemize}
    \item why better than block-based? some elements in autoencoder output are more important than others and the important ones are sometimes put together
    \item why better than interleaving? the elements in autoencoder output have structures that align with tensors, etc. so interleaving may destroy some channels entirely.
\end{itemize}}

Figure~\ref{??} empirically compares these schemes (while fixing other factors, such as packet loss rate and training and testing data).
\jc{Some initial results.}


\subsection{Choice of \rates in autoencoder training}

A desirable autoencoder should fare well under a wide range of \rates, so at first glance, we should simulate as many possible \rate values during training as possible.
Nonetheless, adding too much randomness in \loss may make the training converge more slowly and even to suboptimal autoencoder models. 

It remains an open question how to rigorously pick the best \rates in training.
That said, we try our best to empirically examine different choices of \rates in training.

\jc{
\begin{itemize}
    \item experiment setup
    \item empirical findings: 
    (1) must have zero loss rate
    (2) more \rates doesn't help
\end{itemize}
}



\subsection{Rate adaptation over \newae}

\jc{
\begin{itemize}
    \item explain the rate adaptation logic. how we estimate frame size from complexity
    \item show empirical correlation between complexity and frame size
    \item connect it with rate control in h264.
    \item talk about shared backbone to save memory footprint.
\end{itemize}
}


\subsection{Understanding \newae's loss resilience}

\jc{
\begin{itemize}
    \item \newae's performance is surprising, but can be explained.
    \item flat relationship among elements, no strict hierarchy/dependencies like in svc or fec
    \item saliency is more robust to losses: figure~\ref{fig:per-frame}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/per_frame_quality_degradation_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:per-frame}
\end{figure}


\subsection{Key frame insertion}

\jc{
\begin{itemize}
    \item start with the need for more key frames (more than that in h265).
    \item we "amortize" key frames in different frames. (better also to explain why this isn't possible in h264)
    \item give a simple back-of-envelope estimate of the new size. figure~\ref{fig:keyframe_smooth}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/keyframe_smooth.pdf}
    \caption{}
    \label{fig:keyframe_smooth}
\end{figure}



\section{Real-time video delivery over \newae}

Next, we present the design of \name, a concrete real-time video communication system based on \newae.
In designing \name, we focus primarily on unique issues that arise from using \newae as the codec. 
We group these issues in two categories. 
\begin{packeditemize}
\item First, optimizing the delivery of a single frame to optimize the delay-quality tradeoff. 
\item Second, optimizing the delivery of a sequence of frames when congestion or packet losses persist.
% synchronize the coding/decoding states between the sender and receiver?
\end{packeditemize}


\subsection{Workflow}

Figure~\ref{??} depicts \name's framework, which comprises of three high-level modules: the codec (\newae), the congestion controller, and the transmission controller.
The congestion controller decides the sending rate, and the choice of the congestion control logic is complementary to \newae. 
In \S\ref{??}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{??} or Salsify CC~\cite{??}. 

The transmission controller determines how to packetize \newae coder's output (coded data), deliver the packets, and depacketize all or a subset of packets to the input of \newae's decoder. 
The transmission control module is where \name makes simple yet critical modifications, in order to unleash the full potential of \newae and its data-scalable codec primitive. 
Here, we dive into more details on four major modifications. 
% \jc{we logically separate the system into two level: delivering each single frame and delivering a sequence of frames. }

\jc{emphasize that none of these techniques are exactly new, but the particular design is driven by \newae}

\jc{we don't specify the protocol as they follow naturally from the design and is not our main contribution}


\subsection{Saliency-based redundancy}

Recall from \S\ref{??} that with data-scalable primitive, the quality of a frame depends on the fraction of packets received (under a fixed coder state). 
Thus, it would be ideal to packetize the \newae coder's output in a way that improves the quality when a certain fraction of packets are received.

To this end, \name uses a novel strategy based on the randomization packetization used in \newae training (\S\ref{??}), but optimizes the quality under a given number of packets by leveraging the {\em skew distribution} of high-saliency elements in \newae coded data. 
Here, saliency is defined in the same way as Eq.~\ref{eq:3}, \ie if an element has a high saliency, changing it has a higher impact on the decoded quality than other elements. 
To motive our strategy, we run an analysis across \fillme videos in our dataset and the \newae models of \fillme different quality levels. 
Overall, the sum of saliency of the top \fillme-\fillme\% of elements is higher than the sum of saliency of all remaining elements. \jc{need a few words on why saliency is skewed? will it contradict fig~\ref{fig:per-frame}?}

These skewed distributions of saliency suggest that giving the high-saliency elements more protection can improve decoded quality, even at a cost of slightly more bytes. 
\name employs a simple yet efficient strategy of duplicating the top \fillme\% elements with the highest saliency. 
\jc{more details of the exact strategy}


\subsection{Choosing when to decode a frame}

As new packets arrive at the receiver queue (jitter buffer), the data-scalable primitive offers the receiver in \name a choice; decode now using currently arrived packets or waiting for more packets in hope of improving the quality. 
In contrast, with FEC-based loss-resilient schemes and other H.26x-based schemes (\fillme), the receiver simply has to wait for more packets until the data is decodable. 

\name embraces the primitive of data-scalable coding by carefully trading frame delay with decoded quality. 
When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

This strategy is a well-defined, in sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
\jc{can we also use an illustrative example to help people understand it?}


\subsection{Packet prioritization by sender}


In a WebRTC's sender, retransmitted packets (specified in selective ack) are always prioritized over new packets, simply because selectively retransmitted packets are required by the receiver to decode a prior (reference) frame.\footnote{There are exceptions, such as Salsify which may choose to skip certain frames, but they still prioritize retransmitted packets if the frame they belong to is not skipped.}
However, \name rethinks this seemingly natural choice, and instead prioritize new packets in order to leverage the primitive of data-scalable coding.
The intuitive reason is that a retransmitted packet may not be useful if arrives after the receiver decides to decode the frame. 
In contrast, each packet of a new frame, if delivered, is more likely to arrive before the receiver decodes the new frame and can thus improve its quality. 



\mypara{Extension with multi-path TCP}
\jc{more text}


\subsection{Reference frame synchronization}

An acute reader may have realized an unresolved issue, arising from encoding and decoding being asynchronous. 
If the $(i+1)^{\textrm{th}}$ frame is a P-frame, by default the sender will encode it with the decoded $i^{\textrm{th}}$ frame as the reference (used to compute motion vectors and residuals) with the assumption that the $i^{\textrm{th}}$ was fully received by the receiver. 
Now, if the receiver decodes the $i^{\textrm{th}}$ frame with only a subset of its packets, the P-frame encoding of the $(i+1)^{\textrm{th}}$ frame have a low quality when being decoded with a different reference frame than the encoder has assumed. 

A natural strawman to prevent such quality degradation is always letting the receiver piggyback ``which frame was recently decoded using which packets (just the packet IDs would be sufficient)''. 
With this knowledge, the sender can reconstruct the identical latest frame decoded by the receiver (autoencoder decoding is deterministic), and use this reconstructed frame, rather than the immediate last frame, as the reference of the next P-frame.
However, this means that there will be a non-trivial gap between the reference frame and the frame being encoded, making the P-frame significantly bigger than if the very last frame is used as the reference. 
Such gap between the two frames is usually 3-5 frames (though the exact value depends on the propagation delay), and the P-frames are about \fillme$\times$ bigger. 


To prevent quality degradation with minimum frame size inflation, \name leverages the loss-resilience of \newae. 
Empirically, \newae can tolerate out-of-sync encoding/decoding states for several consecutive frames. 
Figure~\ref{??} \jc{more text}

Inspired by these empirical observations, \name uses a simple logic, referred to as lazy synchronization, to 


% \begin{comment}


% As we have seen, a data-scalable autoencoder is well-suited for connections with dynamic \rates, since its quality is near-optimal under no missing packets but degrade gracefully under higher \rates. 
% While the proposed autoencoders can be functionally integrated in WebRTC or other real-time video platforms by simply replacing the video codec, \name makes several logically simple yet crucial modifications to the video streaming system, to maximally embrace the advantages of data-scalable autoencoders.



% \subsection{Optimizing delivery of individual frames}

% A direct implication of the autoencoder's graceful quality degradation (Figure~\ref{??}) is the ability for the receiver (decoder) to trade delay for quality or vice versa, in a finer granularity than prior solutions. 
% Waiting for one more packet, which may slightly delay the rendering of a frame, always incrementally improve the quality of the frame, allowing the receiver to move along the quality-delay tradeoff in presence of delay/loss of multiple packets.
% In contrast, systems using FEC-based coding have to wait for a certain number of packets, due to the cliff effect (\S\ref{??}) of FEC.

% This property of data-salable autoencoder naturally lands itself to a transport mechanism in between UDP and reliably delivering every packet (or a fixed fraction of packets).
% The example in Figure~\ref{??} illustrates the workflow of how \name determines 



% \jc{
% \begin{itemize}
%     \item on coding a frame: i or p? which ref frame? which model?
%     \item on sending a frame: target sending rate or bitrate?
%     \item on receiving a frame: when to decode a frame?
%     \item on packet loss
% \end{itemize}
% }

% \jc{
% \begin{itemize}
%     \item explain our single-frame delivery module: 
%     \item (1) saliency-based redundancy
%     \item (2) selective retransmission
%     \item (3) multipath tcp extension
%     \item why? plot the impact of zeroing top k values
%     \item compare the original ae vs. new ae
%     \item takeaway: high-impact elements are rare, and impact of each packet is similar
% \end{itemize}
% }



% \subsection{Delivering a sequence of frames}

% \jc{
% \begin{itemize}
%     \item we have to think about long-term effects (propagation effects of \rate)
%     \item (1) packet prioritization in \name: evenly split among new packets.
%     \item contrast it with prioritizing retransmission in webrtc
%     \item (2) \name's way of selecting ref frame (on-demand synchronization)
%     \item explain the tradeoff: always sync-up (high overhead), always not sync-up (low quality)
%     \item empirical result: quality vs. \# of high-\rate frames
%     \item (3) bitrate adaptation: 
% \end{itemize}
% }

% \end{comment}


\section{Implementation}

\name is implemented with \fillme lines of Python (mostly for autoencoder NNs) and \fillme lines of C++ (for frame delivery and WebRTC integration). 
We use the method described in \S\ref{??} to fine-tune \fillme to get \newae's P-frame codec and \fillme to get \newae's I-frame codec. 
The per-packet entropy encoder is implemented by \fillme. 

The code and trained model of \name will be made public upon the publication of this paper.

\mypara{Integration}
The integration with WebRTC is logically straightforward, since \newae (including I-frame and P-frame encodings) exposes very similar interface as the default codec in WebRTC. 
\jc{Ziyi, please fill in the details}

\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}

\mypara{Overhead}
Despite that sharing most NN layers (\S\ref{??}) greatly reduces the memory footprint of the multi-bitrate autoencoders, the compute overhead of autoencoder NNs remains substantial---100ms to encode a frame of \fillme$\times$\fillme on a \fillme GPU (though decoding can be much faster). 
Note that this is already faster than the autoencoder used in a recent work for video streaming.
Fortunately, because \name's autoencoder contains shallow NNs, the encoding and decoding of \newae can be greatly accelerated by OpenVino~\cite{??} and achieve \fillme even on CPUs. 
\jc{kuntai/ziyi, fill in the details here}



% \jc{
% \begin{itemize}
%     \item how to integrate it in webrtc: same logical interface for video coding, packetization. replacing vp8
    
%     \item autoencoder highlight: entropy encoder, i-frame model, p-frame model
    
%     \item use of intel vino to reduce overhead
% \end{itemize}
% }




==> sections/technical_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\newcommand{\Coder}{\ensuremath{C_\phi}\xspace}
\newcommand{\Decoder}{\ensuremath{D_\theta}\xspace}
\newcommand{\Quality}{\ensuremath{F}\xspace}
\newcommand{\Packetize}{\ensuremath{A}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\x}{\ensuremath{\textbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\textbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\textbf{z}}\xspace}
\newcommand{\loss}{\ensuremath{p_{\textrm{loss}}}\xspace}




\section{\newae: Data-Scalable Autoencoder}

\name is a concrete instantiation of data-scalable delivery. 
At a high level, it entails a new data-scalable autoencoder, \newae (presented in this section), and a custom delivery framework that leverages the new autoencoder (discussed in the next section).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

\subsection{Autoencoder background}


We begin with the basic terminology of autoencoders. 
We denote the encoder (a neural network parameterized by weights $\phi$) by $\Coder$ and the decoder (a neural network parameterized by weights $\theta$) by $\Decoder$.
For an input frame $\x$ (a $c\times w\times h$ tensor), the coded data $\z=\Coder(\x)$ will be sent to the receiver, which then runs the decoder to reconstruct the original frame from $\z$: $\hat{\x}=\Decoder(\z)$.
Note that the encoder and decoder perform the lossy compression and are {\em separate} from the lossless entropy coding or FEC coding. (We will discuss entropy encoding and packetization in \S\ref{??}.)

We customize two existing autoencoder architectures, \cite{dvc} for P-frames (with motion vectors and residuals as input) and \cite{qmap} for I-frames (with a static image as input).\footnote{We do not consider B-frames are they are not commonly used in low-latency videos.} 
We borrow their neural network architectures (their architectures in details in \jc{need an appendix on how dvc creates input \x from two frames, and which part of it was trained by us, which part are not.}).
Since they share the same conceptual framework described above, we do not discuss them separately unless necessary.


The compression efficiency of the output $\hat{\x}$ is measured by a function $\Quality(\hat{\x},\x)$, which is a weighted sum of its visual quality (\ie the difference between $\hat{\x}$ and $\x$)\footnote{It is true that pixel-wise distortion is not the best way to capture human perception of compression artifacts, but it is often used in autoencoder training for its differentiability. Our empirical evaluation also shows that the trained autoencoder performs competitively in terms of more standard metrics, such as SSIM and PSNR (both RGB and YUV-based).} and its entropy-coded size (\eg estimated by a pre-trained neural net), with the weight of visual quality being $\alpha$. 
With a higher value of $\alpha$, the trained $\Coder(\x)$ will produce output $\z$ that naturally leads to better visual quality in $\Decoder(\z)$ but higher file size. 
To adapt to the dynamic sending rate, multiple versions of the autoencoders are trained, each with a different weight $\alpha$, and they share most (backbone) layers, which significantly reduces the memory footprint when switching between bitrates. (See \name's bitrate adaptation in \S\ref{??}.) 
% A higher $\Quality$ value is better (higher visual quality and/or lower entropy-coded size).

The fact that $\Coder$, $\Decoder$, and $\Quality$ are differentiable allows end-to-end training of the autoencoder architecture~\cite{??,??,??}.
Mathematically, given a training set $\X$, our goal is 
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\z = \Coder(\x)
\label{eq:1}
\vspace{-0.05cm}
\end{align}

\subsection{Basic formulation of \newae training}

To train a {\em data-scalable autoencoder}, the training process should not only focus on compression efficiency (low bitrate and low reconstruction distortion) but also do so under various packet loss rates.
To this end, we make a few critical changes to the training process of autoencoders.


This traditional training process (Eq.~\ref{eq:1}) can be viewed as having zero packet loss, \ie the input to the decoder is the same as the output of the encoder. 
To incorporate different loss rates, \name proposes a custom training process for autoencoders, by adding a random distribution $\loss$:
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\highlight{blue}{$\z\sim \loss(\z | \Coder(\x))$}
\label{eq:2}
\vspace{-0.05cm}
\end{align}
where the change is highlighted in color.
$\loss$ takes the encoder output $\Coder(\x)$ and returns a distribution over the possible received data seen by the decoder (after packet erasures under non-zero \rate). 
As we will see next, with appropriate randomization, $\loss$ can simulate the effect of packet losses on data received by the decoder.


Simulating packet losses in Eq.~\ref{eq:2} entails three questions:
\begin{packedenumerate}
\item How should $\loss$ convert $\Coder(\x)$ to data packets and change the coded data if packets are randomly dropped? 
%This decides what data seen by the decoder would be if packets are randomly dropped. 
\item Given that the general form of $\loss$ is not differentiable, so how to train autoencoders with Eq.~\ref{eq:2} in presence of the $\loss$ function? 
\item What packet loss rate should be simulated in training, so that the trained model can deal with a range of unseen loss rates?
\end{packedenumerate}
It is important to note that these questions are not involved in canonical autoencoder training, but they become critical here for the need to simulate packet losses in the training process.
% \section{Simulating \rates in autoencoder training}



% \mypara{How to simulate packet losses}

%\mypara{Simulating packet losses in autoencoder training}
%Training a data-scalable autoencoder using Eq.~\ref{eq:2} faces three key questions:
%\begin{packedenumerate}
%\item How to make Eq.~\ref{eq:2} differentiable for a wide range of $\loss$ that simulates various packet loss patterns?
%\item How to convert $\Coder(\x)$ to data packets? This decides how losing a packet would affect the data seen by the decoder.
%\item What \rates should be simulated in training, so that the trained model can deal with a range of unseen \rates?
%\end{packedenumerate}
% The first question concerns packetization of the coder output and the second question concerns what \rates should be used to train the model that can deal with a range of \rates.

% , so that the trained model can handle packet losses of various \rates in real networks. 

\subsection{How to make \newae trainable?}

An immediate challenge imposed by Eq.~\ref{eq:2} is how to train the weights ($\theta$ and $\phi$) of the autoencoder, despite that the random distribution $\loss$ is not a naturally differentiable step. 

% that the expected value of $\Quality$ may not always be written in a closed, differentiable form, so before we discuss how \loss simulate packet losses with a non-zero \rate, we must first be able to run backpropagation for weights $\theta$ and $\phi$ in Eq.~\ref{eq:2}. 


\jc{Yihua/Anton, please explain how you used REINFORCE trick here.
\begin{itemize}
    \item this may look like VAE, so a natural solution is reparameterization. it doesn't work because the expectation of $\Quality$ cannot be writtein in a closed, differentiable form
    \item we use reinforce trick.. how does it work?
\end{itemize}}


\subsection{How to simulate packet losses in autoencoder training?}

\mypara{Packetizing autoencoder output}


\jc{start with how WE do packetization, including per-packet entropy coding, and then list the alternatives}

\jc{an illustration figure here}

As illustrated in Figure~\ref{??} packetization of \name first uses an assignment function $\Packetize$ to map each element of $\z=\Coder(\x)$ to $k$ non-overlapping sublists, and then losslessly encodes each sublist to get the bit stream of a packet.
Conversely, depacketization of \name first losslessly decodes each packet to a sublist and maps the sublists back to $\z$ by the inverse function $\Packetize^{-1}$.
Each packet is numbered so if a packet has not arrived when decoding, the elements mapped it will be set to zero (this is a natural choice, though we will discuss alternatives in \S\ref{??}). 

The key to a good packetization lies in the assignment function $\Packetize$, because it decides how missing one packet would affect the coded data seen by the receiver. 
The lossless coding can use any off-the-shelf entropy coder, and the entropy-encoded bit stream should fit in the size of a packet (1.5KB).
We will discuss our choice of the entropy coder in more details in \S\ref{??}.

We consider three design choices for $\Packetize$:
\begin{packeditemize}
\item Block-based assignment splits $\z$ to {\em contiguous} blocks so elements close together will be encoded in the same packet, much the same way video data is packetized today. 
This serves a reference design point.
\item Interleaving assignment assigns the $i^{\textrm{th}}$ element to the $(i\textrm{ mod }k)^{\textrm{th}}$ packet, where $k$ is the number of packets.
Interleaving-based packetization is recommended by some traditional loss-resilient schemes~\cite{??}.
\item Randomized assignment uses a pseudo-random mapping $\Packetize_{random}$ to assign each element in $\z$ to its position in a packet. 
An inverse function $\Packetize_{random}^{-1}$ (\eg\fillme) can then be used to map the packet data back to $\z$). 
\end{packeditemize}
Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (based on \rates selected in \S\ref{??}). 


\myparaq{Why randomized assignment}
\name chooses randomized assignment over the block-based and the interleaving ones. 
The intuitive reason is that 

\jc{\begin{itemize}
    \item why better than block-based? some elements in autoencoder output are more important than others and the important ones are sometimes put together
    \item why better than interleaving? the elements in autoencoder output have structures that align with tensors, etc. so interleaving may destroy some channels entirely.
\end{itemize}}

Figure~\ref{??} empirically compares these schemes (while fixing other factors, such as packet loss rate and training and testing data).
\jc{Some initial results.}


\subsection{Choice of \rates in autoencoder training}

A desirable autoencoder should fare well under a wide range of \rates, so at first glance, we should simulate as many possible \rate values during training as possible.
Nonetheless, adding too much randomness in \loss may make the training converge more slowly and even to suboptimal autoencoder models. 

It remains an open question how to rigorously pick the best \rates in training.
That said, we try our best to empirically examine different choices of \rates in training.

\jc{
\begin{itemize}
    \item experiment setup
    \item empirical findings: 
    (1) must have zero loss rate
    (2) more \rates doesn't help
\end{itemize}
}



\subsection{Rate adaptation over \newae}

\jc{
\begin{itemize}
    \item explain the rate adaptation logic. how we estimate frame size from complexity
    \item show empirical correlation between complexity and frame size
    \item connect it with rate control in h264.
    \item talk about shared backbone to save memory footprint.
\end{itemize}
}


\subsection{Understanding \newae's loss resilience}

\jc{
\begin{itemize}
    \item \newae's performance is surprising, but can be explained.
    \item flat relationship among elements, no strict hierarchy/dependencies like in svc or fec
    \item saliency is more robust to losses: figure~\ref{fig:per-frame}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/per_frame_quality_degradation_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:per-frame}
\end{figure}


\subsection{Key frame insertion}

\jc{
\begin{itemize}
    \item start with the need for more key frames (more than that in h265).
    \item we "amortize" key frames in different frames. (better also to explain why this isn't possible in h264)
    \item give a simple back-of-envelope estimate of the new size. figure~\ref{fig:keyframe_smooth}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/keyframe_smooth.pdf}
    \caption{}
    \label{fig:keyframe_smooth}
\end{figure}



\section{Real-time video delivery over \newae}

Next, we present the design of \name, a concrete real-time video communication system based on \newae.
In designing \name, we focus primarily on unique issues that arise from using \newae as the codec. 
We group these issues in two categories. 
\begin{packeditemize}
\item First, optimizing the delivery of a single frame to optimize the delay-quality tradeoff. 
\item Second, optimizing the delivery of a sequence of frames when congestion or packet losses persist.
% synchronize the coding/decoding states between the sender and receiver?
\end{packeditemize}


\subsection{Workflow}

Figure~\ref{??} depicts \name's framework, which comprises of three high-level modules: the codec (\newae), the congestion controller, and the transmission controller.
The congestion controller decides the sending rate, and the choice of the congestion control logic is complementary to \newae. 
In \S\ref{??}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{??} or Salsify CC~\cite{??}. 

The transmission controller determines how to packetize \newae coder's output (coded data), deliver the packets, and depacketize all or a subset of packets to the input of \newae's decoder. 
The transmission control module is where \name makes simple yet critical modifications, in order to unleash the full potential of \newae and its data-scalable codec primitive. 
Here, we dive into more details on four major modifications. 
% \jc{we logically separate the system into two level: delivering each single frame and delivering a sequence of frames. }

\jc{emphasize that none of these techniques are exactly new, but the particular design is driven by \newae}

\jc{we don't specify the protocol as they follow naturally from the design and is not our main contribution}


\subsection{Saliency-based redundancy}

Recall from \S\ref{??} that with data-scalable primitive, the quality of a frame depends on the fraction of packets received (under a fixed coder state). 
Thus, it would be ideal to packetize the \newae coder's output in a way that improves the quality when a certain fraction of packets are received.

To this end, \name uses a novel strategy based on the randomization packetization used in \newae training (\S\ref{??}), but optimizes the quality under a given number of packets by leveraging the {\em skew distribution} of high-saliency elements in \newae coded data. 
Here, saliency is defined in the same way as Eq.~\ref{eq:3}, \ie if an element has a high saliency, changing it has a higher impact on the decoded quality than other elements. 
To motive our strategy, we run an analysis across \fillme videos in our dataset and the \newae models of \fillme different quality levels. 
Overall, the sum of saliency of the top \fillme-\fillme\% of elements is higher than the sum of saliency of all remaining elements. \jc{need a few words on why saliency is skewed? will it contradict fig~\ref{fig:per-frame}?}

These skewed distributions of saliency suggest that giving the high-saliency elements more protection can improve decoded quality, even at a cost of slightly more bytes. 
\name employs a simple yet efficient strategy of duplicating the top \fillme\% elements with the highest saliency. 
\jc{more details of the exact strategy}


\subsection{Choosing when to decode a frame}

As new packets arrive at the receiver queue (jitter buffer), the data-scalable primitive offers the receiver in \name a choice; decode now using currently arrived packets or waiting for more packets in hope of improving the quality. 
In contrast, with FEC-based loss-resilient schemes and other H.26x-based schemes (\fillme), the receiver simply has to wait for more packets until the data is decodable. 

\name embraces the primitive of data-scalable coding by carefully trading frame delay with decoded quality. 
When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

This strategy is a well-defined, in sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
\jc{can we also use an illustrative example to help people understand it?}


\subsection{Packet prioritization by sender}


In a WebRTC's sender, retransmitted packets (specified in selective ack) are always prioritized over new packets, simply because selectively retransmitted packets are required by the receiver to decode a prior (reference) frame.\footnote{There are exceptions, such as Salsify which may choose to skip certain frames, but they still prioritize retransmitted packets if the frame they belong to is not skipped.}
However, \name rethinks this seemingly natural choice, and instead prioritize new packets in order to leverage the primitive of data-scalable coding.
The intuitive reason is that a retransmitted packet may not be useful if arrives after the receiver decides to decode the frame. 
In contrast, each packet of a new frame, if delivered, is more likely to arrive before the receiver decodes the new frame and can thus improve its quality. 



\mypara{Extension with multi-path TCP}
\jc{more text}


\subsection{Reference frame synchronization}

An acute reader may have realized an unresolved issue, arising from encoding and decoding being asynchronous. 
If the $(i+1)^{\textrm{th}}$ frame is a P-frame, by default the sender will encode it with the decoded $i^{\textrm{th}}$ frame as the reference (used to compute motion vectors and residuals) with the assumption that the $i^{\textrm{th}}$ was fully received by the receiver. 
Now, if the receiver decodes the $i^{\textrm{th}}$ frame with only a subset of its packets, the P-frame encoding of the $(i+1)^{\textrm{th}}$ frame have a low quality when being decoded with a different reference frame than the encoder has assumed. 

A natural strawman to prevent such quality degradation is always letting the receiver piggyback ``which frame was recently decoded using which packets (just the packet IDs would be sufficient)''. 
With this knowledge, the sender can reconstruct the identical latest frame decoded by the receiver (autoencoder decoding is deterministic), and use this reconstructed frame, rather than the immediate last frame, as the reference of the next P-frame.
However, this means that there will be a non-trivial gap between the reference frame and the frame being encoded, making the P-frame significantly bigger than if the very last frame is used as the reference. 
Such gap between the two frames is usually 3-5 frames (though the exact value depends on the propagation delay), and the P-frames are about \fillme$\times$ bigger. 


To prevent quality degradation with minimum frame size inflation, \name leverages the loss-resilience of \newae. 
Empirically, \newae can tolerate out-of-sync encoding/decoding states for several consecutive frames. 
Figure~\ref{??} \jc{more text}

Inspired by these empirical observations, \name uses a simple logic, referred to as lazy synchronization, to 


% \begin{comment}


% As we have seen, a data-scalable autoencoder is well-suited for connections with dynamic \rates, since its quality is near-optimal under no missing packets but degrade gracefully under higher \rates. 
% While the proposed autoencoders can be functionally integrated in WebRTC or other real-time video platforms by simply replacing the video codec, \name makes several logically simple yet crucial modifications to the video streaming system, to maximally embrace the advantages of data-scalable autoencoders.



% \subsection{Optimizing delivery of individual frames}

% A direct implication of the autoencoder's graceful quality degradation (Figure~\ref{??}) is the ability for the receiver (decoder) to trade delay for quality or vice versa, in a finer granularity than prior solutions. 
% Waiting for one more packet, which may slightly delay the rendering of a frame, always incrementally improve the quality of the frame, allowing the receiver to move along the quality-delay tradeoff in presence of delay/loss of multiple packets.
% In contrast, systems using FEC-based coding have to wait for a certain number of packets, due to the cliff effect (\S\ref{??}) of FEC.

% This property of data-salable autoencoder naturally lands itself to a transport mechanism in between UDP and reliably delivering every packet (or a fixed fraction of packets).
% The example in Figure~\ref{??} illustrates the workflow of how \name determines 



% \jc{
% \begin{itemize}
%     \item on coding a frame: i or p? which ref frame? which model?
%     \item on sending a frame: target sending rate or bitrate?
%     \item on receiving a frame: when to decode a frame?
%     \item on packet loss
% \end{itemize}
% }

% \jc{
% \begin{itemize}
%     \item explain our single-frame delivery module: 
%     \item (1) saliency-based redundancy
%     \item (2) selective retransmission
%     \item (3) multipath tcp extension
%     \item why? plot the impact of zeroing top k values
%     \item compare the original ae vs. new ae
%     \item takeaway: high-impact elements are rare, and impact of each packet is similar
% \end{itemize}
% }



% \subsection{Delivering a sequence of frames}

% \jc{
% \begin{itemize}
%     \item we have to think about long-term effects (propagation effects of \rate)
%     \item (1) packet prioritization in \name: evenly split among new packets.
%     \item contrast it with prioritizing retransmission in webrtc
%     \item (2) \name's way of selecting ref frame (on-demand synchronization)
%     \item explain the tradeoff: always sync-up (high overhead), always not sync-up (low quality)
%     \item empirical result: quality vs. \# of high-\rate frames
%     \item (3) bitrate adaptation: 
% \end{itemize}
% }

% \end{comment}


\section{Implementation}

\name is implemented with \fillme lines of Python (mostly for autoencoder NNs) and \fillme lines of C++ (for frame delivery and WebRTC integration). 
We use the method described in \S\ref{??} to fine-tune \fillme to get \newae's P-frame codec and \fillme to get \newae's I-frame codec. 
The per-packet entropy encoder is implemented by \fillme. 

The code and trained model of \name will be made public upon the publication of this paper.

\mypara{Integration}
The integration with WebRTC is logically straightforward, since \newae (including I-frame and P-frame encodings) exposes very similar interface as the default codec in WebRTC. 
\jc{Ziyi, please fill in the details}

\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}

\mypara{Overhead}
Despite that sharing most NN layers (\S\ref{??}) greatly reduces the memory footprint of the multi-bitrate autoencoders, the compute overhead of autoencoder NNs remains substantial---100ms to encode a frame of \fillme$\times$\fillme on a \fillme GPU (though decoding can be much faster). 
Note that this is already faster than the autoencoder used in a recent work for video streaming.
Fortunately, because \name's autoencoder contains shallow NNs, the encoding and decoding of \newae can be greatly accelerated by OpenVino~\cite{??} and achieve \fillme even on CPUs. 
\jc{kuntai/ziyi, fill in the details here}



% \jc{
% \begin{itemize}
%     \item how to integrate it in webrtc: same logical interface for video coding, packetization. replacing vp8
    
%     \item autoencoder highlight: entropy encoder, i-frame model, p-frame model
    
%     \item use of intel vino to reduce overhead
% \end{itemize}
% }




==> sections/technical_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\newcommand{\Coder}{\ensuremath{C_\phi}\xspace}
\newcommand{\Decoder}{\ensuremath{D_\theta}\xspace}
\newcommand{\Quality}{\ensuremath{F}\xspace}
\newcommand{\Packetize}{\ensuremath{A}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\x}{\ensuremath{\textbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\textbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\textbf{z}}\xspace}
\newcommand{\loss}{\ensuremath{p_{\textrm{loss}}}\xspace}




\section{\newae: Data-Scalable Autoencoder}

\name is a concrete instantiation of data-scalable delivery. 
At a high level, it entails a new data-scalable autoencoder, \newae (presented in this section), and a custom delivery framework that leverages the new autoencoder (discussed in the next section).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

\subsection{Autoencoder background}


We begin with the basic terminology of autoencoders. 
We denote the encoder (a neural network parameterized by weights $\phi$) by $\Coder$ and the decoder (a neural network parameterized by weights $\theta$) by $\Decoder$.
For an input frame $\x$ (a $c\times w\times h$ tensor), the coded data $\z=\Coder(\x)$ will be sent to the receiver, which then runs the decoder to reconstruct the original frame from $\z$: $\hat{\x}=\Decoder(\z)$.
Note that the encoder and decoder perform the lossy compression and are {\em separate} from the lossless entropy coding or FEC coding. (We will discuss entropy encoding and packetization in \S\ref{??}.)

We customize two existing autoencoder architectures, \cite{dvc} for P-frames (with motion vectors and residuals as input) and \cite{qmap} for I-frames (with a static image as input).\footnote{We do not consider B-frames are they are not commonly used in low-latency videos.} 
We borrow their neural network architectures (their architectures in details in \jc{need an appendix on how dvc creates input \x from two frames, and which part of it was trained by us, which part are not.}).
Since they share the same conceptual framework described above, we do not discuss them separately unless necessary.


The compression efficiency of the output $\hat{\x}$ is measured by a function $\Quality(\hat{\x},\x)$, which is a weighted sum of its pixel-distortion $Distortion(\hat{\x},\x)$, (\ie the difference between $\hat{\x}$ and $\x$)\footnote{It is true that pixel-wise distortion is not the best way to capture human perception of compression artifacts, but it is often used in autoencoder training for its differentiability. Our empirical evaluation also shows that the trained autoencoder performs competitively in terms of more standard metrics, such as SSIM and PSNR (both RGB and YUV-based).} and its entropy-encoded size $Size(\hat{x})$ (\eg estimated by a pre-trained neural net), with the weight of size being $\alpha$: $\Quality(\hat{\x},\x)= Distortion(\hat{\x},\x)+\alpha\cdot Size(\hat{\x})$
With a higher value of $\alpha$, the trained $\Coder(\x)$ will produce output $\z$ that naturally leads to better visual quality in $\Decoder(\z)$ but higher file size. 
To adapt to the dynamic sending rate, multiple versions of the autoencoders are trained, each with a different weight $\alpha$, and they share most (backbone) layers, which significantly reduces the memory footprint when switching between bitrates. (See \name's bitrate adaptation in \S\ref{??}.) 
% A higher $\Quality$ value is better (higher visual quality and/or lower entropy-coded size).

The fact that $\Coder$, $\Decoder$, and $\Quality$ are differentiable allows end-to-end training of the autoencoder architecture~\cite{??,??,??}.
Mathematically, given a training set $\X$, our goal is 
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\z = \Coder(\x)
\label{eq:1}
\vspace{-0.05cm}
\end{align}

\jc{anton/yihua, can you draw a simplified figure to depict the input/output of the used autoencoders? the figure should also include the tensor dimensions of the input and output. }

\subsection{Basic formulation of \newae training}

To train a {\em data-scalable autoencoder}, the training process should not only focus on compression efficiency (low bitrate and low reconstruction distortion) but also do so under various packet loss rates.
To this end, we make a few critical changes to the training process of autoencoders.


This traditional training process (Eq.~\ref{eq:1}) can be viewed as having zero packet loss, \ie the input to the decoder is the same as the output of the encoder. 
To incorporate different loss rates, \name proposes a custom training process for autoencoders, by adding a random distribution $\loss$:
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\highlight{blue}{$\z\sim \loss(\z | \Coder(\x))$}
\label{eq:2}
\vspace{-0.05cm}
\end{align}
where the change is highlighted in color.
$\loss$ takes the encoder output $\Coder(\x)$ and returns a distribution over the possible received data seen by the decoder (after packet erasures under non-zero \rate). 
As we will see next, with appropriate randomization, $\loss$ can simulate the effect of packet losses on data received by the decoder.


Simulating packet losses in Eq.~\ref{eq:2} entails three questions, which we will address in the remaining of this section.
\begin{packedenumerate}
\item How should $\loss$ convert $\Coder(\x)$ to data packets and change the coded data if packets are randomly dropped (\S\ref{subsec:sim-losses})? 
%This decides what data seen by the decoder would be if packets are randomly dropped. 
\item Given that the general form of $\loss$ is not differentiable, so how to train autoencoders with Eq.~\ref{eq:2} in presence of the $\loss$ function (\S\ref{subsec:sim-trainable})? 
\item What packet loss rate should be simulated in training, so that the trained model can deal with a range of unseen loss rates (\S\ref{subsec:sim-lossrate})?
\end{packedenumerate}
It is important to note that these questions are not involved in canonical autoencoder training, but they become critical here for the need to simulate packet losses in the training process.
% \section{Simulating \rates in autoencoder training}



% \mypara{How to simulate packet losses}

%\mypara{Simulating packet losses in autoencoder training}
%Training a data-scalable autoencoder using Eq.~\ref{eq:2} faces three key questions:
%\begin{packedenumerate}
%\item How to make Eq.~\ref{eq:2} differentiable for a wide range of $\loss$ that simulates various packet loss patterns?
%\item How to convert $\Coder(\x)$ to data packets? This decides how losing a packet would affect the data seen by the decoder.
%\item What \rates should be simulated in training, so that the trained model can deal with a range of unseen \rates?
%\end{packedenumerate}
% The first question concerns packetization of the coder output and the second question concerns what \rates should be used to train the model that can deal with a range of \rates.

% , so that the trained model can handle packet losses of various \rates in real networks. 



\subsection{Simulating packet losses over autoencoders}
\label{subsec:sim-losses}

To simulate the impact of losing a packet, we first explain how \name packetizes the encoder output $\z=\Coder(\x)$.

\jc{an illustration figure here}

As illustrated in Figure~\ref{??}, \name first uses a {\em packetization function} $\Packetize$ to map each element position in $\z=\Coder(\x)$ (a 3-D or 4-D tensor) to $k$ non-overlapping lists (\name uses \fillme) and then losslessly encodes the elements in each list to produce the bitstream of a packet.\footnote{It is important to note that \name's {\em per-packet} entropy coding makes each packets individually decodable. 
This is different from typical autoencoders which entropy encodes the whole $\z$ tensor before packetization and thus any lost packet will make the received data not decodable by the entropy decoder. 
Moreover, since we use arithmetic coding (\fillme), so the total size of individually encoded packets is similar to the output of coding $\z$, if the elements in each packet share the same distribution as all elements in $\z$ (which is fortuitously ensured by random mapping). 
}
Conversely, depacketization in \name first losslessly decodes each packet to a list of elements and maps element back to their original positions in $\z$ by the inverse function $\Packetize^{-1}$.
One can use an off-the-shelf entropy coder to losslessly code the elements in a packet to a bitstream. (We discuss in \S\ref{??} \jc{need an appendix here} how to fit the bitstream in the normal packet size of 1.4KB.)


If a packet is lost, each element whose position is mapped by $\Packetize$ to the lost packet will be set to zero (this is a natural choice, though there are alternatives, which will be discussed in \S\ref{??}). 
 The choice of the packetization function $\Packetize$ is thus critical, since it decides how missing one packet would affect the coded data seen by the receiver.  
\name's packetization function is a {\em random} mapping; specifically, the pseudo-random function \fillme which has a reverse mapping. 
As a result, if the random packet loss rate is 30\%, then $\loss(\z|\Coder(\x))$ will produce a distribution of $\z$ that result from randomly setting 30\% of elements in $\z$ to be zeros. 

The use of randomized packetization seems straightforward, but it empirically works better than alternatives, for two reasons. 
\begin{packeditemize}
\item Some elements in autoencoder output $\z$ are more important than others (see \S\ref{??} for some examples), and zeroing each important element has disproportionally higher impact on the decoded quality than zeroing other elements.
A random mapping makes sure that losing $x\%$ packets will affect $x\%$ important elements (whereas a non-randomized packetization may affect more than $x\%$ important elements).
\item A random mapping ensures that all elements in $\z$ has the same distribution as those mapped to each packet. This makes it easier to maintain roughly same entropy-encoded size of each packet. 
\end{packeditemize}

In \S\ref{subsec:??}, we will empirically compare \newae trained with the random packetization and \newae trained with some alternative packetization schemes, such as block-based packetization (\ie each packet contains a contiguous block of elements in $\z$) and interleaving-based packetization. 
Both are suboptimal, since important elements can be next to each other and have a fixed distance with each other under $\z$'s specific tensor structure, so in the worst case both block-based packetization and interleaving packetization can drop higher fraction of important elements than packet loss rate.



%\name uses a {\em random} mapping $\Packetize_{random}$ 
%
%This choice of  $\Packetize$ is driven by two reasons. 
%An inverse function $\Packetize_{random}^{-1}$ (\eg\fillme) can then be used to map the packet data back to $\z$). 
%Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (we will discuss the choice of packet loss rates used in training shortly). 
%Each packet is numbered so if a packet has not arrived when decoding, the elements mapped to it will be set to zero (this is a natural choice, though we will discuss alternatives in \S\ref{??}). 
%
%%\jc{start with how WE do packetization, including per-packet entropy coding, and then list the alternatives}
%
%We compare the choice of random assignment with two strawmen:
%\begin{packeditemize}
%\item Block-based assignment splits $\z$ to {\em contiguous} blocks so elements close together will be encoded in the same packet, much the same way video data is packetized today. 
%This serves a reference design point.
%\item Interleaving assignment assigns the $i^{\textrm{th}}$ element to the $(i\textrm{ mod }k)^{\textrm{th}}$ packet, where $k$ is the number of packets.
%Interleaving-based packetization is recommended by some traditional loss-resilient schemes~\cite{??}.
%\end{packeditemize}
%Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (based on \rates selected in \S\ref{??}). 


%\myparaq{Why randomized assignment}
%\name chooses randomized assignment over the block-based and the interleaving ones. 
%The intuitive reason is that 
%
%\jc{\begin{itemize}
%\item why better than block-based? some elements in autoencoder output are more important than others and the important ones are sometimes put together
%\item why better than interleaving? the elements in autoencoder output have structures that align with tensors, etc. so interleaving may destroy some channels entirely.
%\end{itemize}}
%
%Figure~\ref{??} empirically compares these schemes (while fixing other factors, such as packet loss rate and training and testing data).
%\jc{Some initial results.}



\subsection{How to make \newae trainable?}
\label{subsec:sim-trainable}

Next, we need to make Eq.~\ref{eq:2} trainable for the weights ($\theta$ and $\phi$) when $\loss$ is a random function. 
%A challenge imposed by Eq.~\ref{eq:2} is how to train the weights ($\theta$ and $\phi$) of the autoencoder, despite that the random distribution $\loss$ is not a naturally differentiable step. 

% that the expected value of $\Quality$ may not always be written in a closed, differentiable form, so before we discuss how \loss simulate packet losses with a non-zero \rate, we must first be able to run backpropagation for weights $\theta$ and $\phi$ in Eq.~\ref{eq:2}. 


\jc{Yihua/Anton, please explain how you used REINFORCE trick here.
\begin{itemize}
    \item this may look like VAE, so a natural solution is reparameterization. it doesn't work because the expectation of $\Quality$ cannot be writtein in a closed, differentiable form
    \item we use reinforce trick.. how does it work?
\end{itemize}}

\subsection{Choice of packet loss rate in training}
\label{subsec:sim-lossrate}

As the packet loss rate varies over time, a desirable autoencoder should fare well under unseen packet loss rates.
We acknowledge that it remains an open question what packet loss rates should be used to train \newae to obtain ideal generalization under unseen packet loss rates. 
But we try our best to explore different strategies of setting packet loss rates. 

At first glance, we should simulate as many packet loss rates during training as possible.
However, we found that adding too much randomness in \loss might make the training converge more slowly and even to suboptimal autoencoder models. 
Specifically, our empirical results show that (1) training \newae with just a few values of packet loss rates generalizes better than with a wide range of packet loss rates, even on unseen test packet loss rates, and (2) the packet loss rates in training should include 0\% (otherwise the trained autoencoder will perform significantly worse than the pre-trained autoencoder on low packet loss rates. 

\jc{yihua/anton, please add a figure here to compare psnr-vs-loss under different training loss distributions}

To illustrate them, Figure~\ref{??} compares three choices of training packet loss rates.
\begin{packeditemize}
\item {\em Distribution-1:} \fillme
\item {\em Distribution-2:} \fillme
\item {\em Distribution-3:} \fillme
\end{packeditemize}
\name uses Distribution-1. 
\jc{yihua/anton, please fill in a short para on the read of the figure}

The intuition that more training packet loss rates might not help is that \fillme

%\jc{
%\begin{itemize}
%    \item experiment setup
%    \item empirical findings: 
%    (1) must have zero loss rate
%    (2) more \rates doesn't help
%\end{itemize}
%}


\subsection{Understanding \newae's loss resilience}

As illustrated in Figure~\ref{fig:autoencoder-pretrained}, compared to the pre-trained autoencoder (which is already data-scalable), \newae (re-trained on the same video dataset but with packet losses) achieves much higher quality on unseen videos under various test packet loss rates, even those that are {\em not} seen during training. 
This remarkable improvement begs the question why \newae can be much more resilient to packet losses. We believe that the reasons are two-fold. 


First, compared to SVC, FEC or H.26x-based coding, the elements in \newae's encoding output (before entropy encoding) does not impose any strict structure (\eg hierarchy or dependencies). 
Instead, the relationship between elements in \newae output is ``flat'', and changing any element (to zeo) would not render the frame non-decodable. 

Second, compared to the pre-trained autoencoder, the custom training process described in \S\ref{??} reduces the sensitivity of decoding quality to individual elements.
Though this effect is hard to directly show, we can illustrate it as follows.
We first calculate the ``gradient'' of decoding quality with respect to each element in $\z$ (defined shortly).
Mathematically, the gradient of decoding quality with respect to elements in $\z$ is a vector:
\vspace{-0.05cm}
\begin{align}
\vec{g}=\frac{\partial \Quality(\Decoder(\z),\x)}{\partial\z}
\vspace{-0.05cm}
\end{align}
Figure~\ref{fig:per-frame} shows the incremental impact on decoding quality if more elements are zeroed in descending order of the gradient.
As more elements are zeroed, we can see that quality of the pre-trained autoencoder drops sharply, whereas that of \newae drops much more slowly. 



%\jc{
%\begin{itemize}
%    \item \newae's performance is surprising, but can be explained.
%    \item flat relationship among elements, no strict hierarchy/dependencies like in svc or fec
%    \item saliency is more robust to losses: figure~\ref{fig:per-frame}
%\end{itemize}
%}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/per_frame_quality_degradation_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:per-frame}
\end{figure}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.92\linewidth]{figs/transmission_overview.pdf}
    \caption{}
    \label{fig:overview}
\end{figure*}


\section{Real-time video delivery over \newae}

\name is a concrete real-time video communication system built on a data-scalable autoencoder (\newae).
In designing \name, we focus primarily on unique issues  arising from the use of \newae as the codec, including how to delivery each frame to strike a desirable delay-quality tradeoff (without skipping frames), and how to delivery a sequence of frames when congestion or packet losses affect multiple frames. 
%We group these issues in two categories. 
%\begin{packeditemize}
%\item First, optimizing the delivery of a single frame to optimize the delay-quality tradeoff. 
%\item Second, optimizing the delivery of a sequence of frames when congestion or packet losses persist.
%% synchronize the coding/decoding states between the sender and receiver?
%\end{packeditemize}


%\mypara{Workflow and modules}
Figure~\ref{fig:overview} depicts \name's framework, which comprises of three high-level modules: the codec (\newae), the congestion controller, and the transmission controller.
The congestion controller decides the sending rate, and the choice of the congestion control logic is complementary to \newae. 
In \S\ref{??}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{??} or Salsify CC~\cite{??}. 

The transmission controller determines how to packetize \newae coder's output (coded data), deliver the packets, and depacketize all or a subset of packets to the input of \newae's decoder. 
Other than the codec (\newae), most \name's changes are made in the transmission module. 
We do not claim that any of the modifications is exactly new (\eg a variant of reference frame synchronization has been used in~\cite(salsify)). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \newae and its data-scalable codec primitive.

% \jc{we logically separate the system into two level: delivering each single frame and delivering a sequence of frames. }

Here, we highlight on on four major modifications (more optimizations are discussed in \S\ref{??}).

%\jc{we don't specify the protocol as they follow naturally from the design and is not our main contribution}

\begin{comment}
\subsection{Saliency-based redundancy}

Recall from \S\ref{??} that with data-scalable primitive, the quality of a frame depends on the fraction of packets received (under a fixed coder state). 
Thus, it would be ideal to packetize the \newae coder's output in a way that improves the quality when a certain fraction of packets are received.

To this end, \name uses a novel strategy based on the randomization packetization used in \newae training (\S\ref{??}), but optimizes the quality under a given number of packets by leveraging the {\em skew distribution} of high-saliency elements in \newae coded data. 
Here, saliency is defined in the same way as Eq.~\ref{eq:3}, \ie if an element has a high saliency, changing it has a higher impact on the decoded quality than other elements. 
To motive our strategy, we run an analysis across \fillme videos in our dataset and the \newae models of \fillme different quality levels. 
Overall, the sum of saliency of the top \fillme-\fillme\% of elements is higher than the sum of saliency of all remaining elements. \jc{need a few words on why saliency is skewed? will it contradict fig~\ref{fig:per-frame}?}

These skewed distributions of saliency suggest that giving the high-saliency elements more protection can improve decoded quality, even at a cost of slightly more bytes. 
\name employs a simple yet efficient strategy of duplicating the top \fillme\% elements with the highest saliency. 
\jc{more details of the exact strategy}

\end{comment}

\subsection{Choosing when to decode a frame}

As new packets arrive at the receiver queue (the internal jitter buffer), the data-scalable abstraction allows the receiver to flexibly decide whether to decode the frame now using currently arrived packets or waiting for more packets in hope of improving the quality. 
In contrast, with FEC-based loss-resilient schemes and other H.26x-based schemes (\fillme), the receiver simply has to wait for more packets until the data is decodable. 

\name embraces this flexibility by carefully trading frame delay with decoded quality. 
When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

\jc{Ziyi and Hanchen: please add a nice description of your logic here}

This strategy is a well-defined, in sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
\jc{can we also use an illustrative example to help people understand it?}


\subsection{Packet scheduling by sender}

\jc{need to discuss it}

In a WebRTC's sender, retransmitted packets (specified in selective/negative acks) are always prioritized over new packets, simply because selectively retransmitted packets are required by the receiver to decode a prior (reference) frame. %\footnote{Exceptions exist, \eg Salsify may skip certain frames.}
\name rethinks this seemingly natural choice, and instead prioritizes new packets in order to leverage data-scalable delivery.
The reason is that a receiver in \name can decode anytime after it receives the first packet, so a retransmitted packet may not be useful if it arrives after the frame is already decoded. 
On the other hand, each packet of a new frame, if delivered, is more likely to arrive before the receiver decodes the new frame and can thus improve its quality. 

To make it work, the sender and the receiver be aware of the other's decision, regarding whether a previous frame's packets are still being resent or 



%\mypara{Extension with multi-path TCP}
%\jc{more text}


\subsection{Reference frame synchronization}

\jc{need to discuss it}

An acute reader may have realized an unresolved issue, arising from encoding and decoding being asynchronous. 
If the $(i+1)^{\textrm{th}}$ frame is a P-frame, by default the sender will encode it with the decoded $i^{\textrm{th}}$ frame as the reference (used to compute motion vectors and residuals) with the assumption that the $i^{\textrm{th}}$ was fully received by the receiver. 
Now, if the receiver decodes the $i^{\textrm{th}}$ frame with only a subset of its packets, the P-frame encoding of the $(i+1)^{\textrm{th}}$ frame have a low quality when being decoded with a different reference frame than the encoder has assumed. 

A natural strawman to prevent such quality degradation is always letting the receiver piggyback ``which frame was recently decoded using which packets (just the packet IDs would be sufficient)''. 
With this knowledge, the sender can reconstruct the identical latest frame decoded by the receiver (autoencoder decoding is deterministic), and use this reconstructed frame, rather than the immediate last frame, as the reference of the next P-frame.
However, this means that there will be a non-trivial gap between the reference frame and the frame being encoded, making the P-frame significantly bigger than if the very last frame is used as the reference. 
Such gap between the two frames is usually 3-5 frames (though the exact value depends on the propagation delay), and the P-frames are about \fillme$\times$ bigger. 


To prevent quality degradation with minimum frame size inflation, \name leverages the loss-resilience of \newae. 
Empirically, \newae can tolerate out-of-sync encoding/decoding states for several consecutive frames. 
Figure~\ref{??} \jc{more text}

Inspired by these empirical observations, \name uses a simple logic, referred to as lazy synchronization, to 


% \begin{comment}


% As we have seen, a data-scalable autoencoder is well-suited for connections with dynamic \rates, since its quality is near-optimal under no missing packets but degrade gracefully under higher \rates. 
% While the proposed autoencoders can be functionally integrated in WebRTC or other real-time video platforms by simply replacing the video codec, \name makes several logically simple yet crucial modifications to the video streaming system, to maximally embrace the advantages of data-scalable autoencoders.



% \subsection{Optimizing delivery of individual frames}

% A direct implication of the autoencoder's graceful quality degradation (Figure~\ref{??}) is the ability for the receiver (decoder) to trade delay for quality or vice versa, in a finer granularity than prior solutions. 
% Waiting for one more packet, which may slightly delay the rendering of a frame, always incrementally improve the quality of the frame, allowing the receiver to move along the quality-delay tradeoff in presence of delay/loss of multiple packets.
% In contrast, systems using FEC-based coding have to wait for a certain number of packets, due to the cliff effect (\S\ref{??}) of FEC.

% This property of data-salable autoencoder naturally lands itself to a transport mechanism in between UDP and reliably delivering every packet (or a fixed fraction of packets).
% The example in Figure~\ref{??} illustrates the workflow of how \name determines 



% \jc{
% \begin{itemize}
%     \item on coding a frame: i or p? which ref frame? which model?
%     \item on sending a frame: target sending rate or bitrate?
%     \item on receiving a frame: when to decode a frame?
%     \item on packet loss
% \end{itemize}
% }

% \jc{
% \begin{itemize}
%     \item explain our single-frame delivery module: 
%     \item (1) saliency-based redundancy
%     \item (2) selective retransmission
%     \item (3) multipath tcp extension
%     \item why? plot the impact of zeroing top k values
%     \item compare the original ae vs. new ae
%     \item takeaway: high-impact elements are rare, and impact of each packet is similar
% \end{itemize}
% }



% \subsection{Delivering a sequence of frames}

% \jc{
% \begin{itemize}
%     \item we have to think about long-term effects (propagation effects of \rate)
%     \item (1) packet prioritization in \name: evenly split among new packets.
%     \item contrast it with prioritizing retransmission in webrtc
%     \item (2) \name's way of selecting ref frame (on-demand synchronization)
%     \item explain the tradeoff: always sync-up (high overhead), always not sync-up (low quality)
%     \item empirical result: quality vs. \# of high-\rate frames
%     \item (3) bitrate adaptation: 
% \end{itemize}
% }

% \end{comment}


\section{Implementation}

\name is implemented with \fillme lines of Python (mostly for autoencoder NNs) and \fillme lines of C++ (for frame delivery and WebRTC integration).\footnote{The code and trained model of \name will be made public upon the publication of this paper.} 
We use the method described in \S\ref{??} to fine-tune \fillme~\cite{??} to get \newae's P-frame codec and \fillme~\cite{??} to get \newae's I-frame codec. 
The per-packet entropy encoding uses \fillme~\cite{??}. 



\subsection{Integration with WebRTC}
The integration with WebRTC is logically straightforward, since \newae (including I-frame and P-frame encodings) exposes very similar interface as the default codec in WebRTC. 
\jc{Ziyi, please fill in the details}

\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}




\subsection{Optimizations}

While autoencoders are functionally similar to traditional codec (so is \newae), they face a few technical challenges to function as the codec in a real-time video client.
Note that these challenges are not unique to loss resilience, so we do not consider packet losses in the rest of the section. 


\mypara{Key frame insertion}
For the P-frame autoencoder we have tried, we observe that the decoded quality can be very high right after each I-frame but it gradually degrades after about 10 frames. 
A naive solution would be to encode an I-frame very often (say once every 10 frames).
This is obviously not ideal, because the I-frames are much larger than P-frames and sending a large frame frequently and a handful of small frames in between can cause great difficulties for congestion control and bitrate adaptation (which will be discussed shortly).\footnote{We have observed that many computer-vision papers on autoencoders have conveniently used a small GoP when compared against H.265, but the implication of large I-frame size for congestion control is rarely discussed.}

Instead of adding new I-frame frequently, \name encodes a small patch (about \fillme$\times$\fillme) as a tiny I-frame on {\em every frame} (the pixels outside the patch will be encoded as a P-frame), and the location of the patch on a frame changes, such that every $k$ frames, the patch will scan through the whole frame size. 
This scheme effectively ``amortizes'' the size of I-frames across $k$ P-frames, as illustrated in Figure~\ref{fig:keyframe_smooth}.
As a result, the frame size will have much lower variance than if I-frames are encoded entirely and inserted intermittently.

%\jc{
%\begin{itemize}
%    \item start with the need for more key frames (more than that in h265).
%    \item we "amortize" key frames in different frames. (better also to explain why this isn't possible in h264)
%    \item give a simple back-of-envelope estimate of the new size. figure~\ref{fig:keyframe_smooth}
%\end{itemize}
%}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/keyframe_smooth.pdf}
    \caption{}
    \label{fig:keyframe_smooth}
\end{figure}


%A client must be able to encode each frame at a given target size. 
\mypara{Encoding at multiple bitrates}
In real-time video, throughput estimation can vary even between two consecutive frames.
Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 


\name provides a similar mechanism. 
First, it trains multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{3.1}).
The resulting autoencoders cover a bitrate range \fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should select the autoencoder whose encoded frame size is lower than the target. 

\jc{need a figure here}

\mypara{Bitrate adaptation} 
To select an autoencoder with frame size lower than the target, we leverage an empirical property of these autoencoders (illustrated in Figure~\ref{??}): 
for each pair of a high-bitrate autoencoder (trained with a high $\alpha$) and a low-bitrate autoencoder (trained with a low $\alpha$), if we denote their encoded frame sizes on the same frame are $S_h$ and $S_l$, then $S_h/S_l$ is roughly constant, despite both $S_h$ and $S_l$ vary between frames. 
Thus, each time when a frame is encoded by one autoencoder, \name can then infer the frame size of other autoencoders on the same frame.
This information can be used to correct the estimated frame size of each autoencoder on current frames. 
This logic is similar to the rate control logic in H.264, which corrects the bitrate estimation based on the latest encoded frame sizes.


\mypara{Reducing memory footprint}
For the client to switch between multiple autoencoders (with different bitrates), their memory footprint in should be minimized, so more of them can be loaded in GPU memory to avoid delay of loading and unloading models. 
\name trains multiple autoencoders by fine-tuning the last 10-25\% layers of the same model (\ie they share the backbone layers), so only the one autoencoder and the last few layers of different autoencoders need to be loaded in GPU memory. 
This reduces the memory footprint of the models by \fillme\% compared to when all models are trained separately without sharing any layers.
A similar idea has also been used in Swift~\cite{swift} to reduce memory usage of multiple SVC layer encoders, though \name uses it to reduce memory footprint of data-scalable autoencoders of different bitrates.\footnote{A note on I-frames}


%\jc{
%\begin{itemize}
%    \item explain the rate adaptation logic. how we estimate frame size from complexity
%    \item show empirical correlation between complexity and frame size
%    \item connect it with rate control in h264.
%    \item talk about shared backbone to save memory footprint.
%\end{itemize}
%}


%\mypara{Reducing system overhead}
%Despite that sharing most NN layers (\S\ref{??}) greatly reduces the memory footprint of the multi-bitrate autoencoders, the compute overhead of autoencoder NNs remains substantial---100ms to encode a frame of \fillme$\times$\fillme on a \fillme GPU (though decoding can be much faster). 
%Note that this is already faster than the autoencoder used in a recent work for video streaming.
%Fortunately, because \name's autoencoder contains shallow NNs, the encoding and decoding of \newae can be greatly accelerated by OpenVino~\cite{??} and achieve \fillme even on CPUs. 
%\jc{kuntai/ziyi, fill in the details here}


\mypara{Reducing compute overhead}
Most research on autoencoder focuses on coding efficiency (using less bits to get higher quality), and the encoding, including \name's implementation, is usually slower than heavily engineered codecs like H.265.
That said, we show that \name's encoding speed can be greatly sped up and achieve an acceptable speed on typical commercial GPUs: from 5~fps on 720p HD (and \fillme~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and \fillme~fps) on a single \$\fillme NVIDIA GeForce 3080 GPU). More results in \S\ref{??}. 

\name achieves such speedup by downsizing the image (by default $4\times$) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
This significantly speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding but their delay is proportional to the input dimension. 
At the same time, because the residuals are still computed between the full-resolution frame and the motion-compensated image, the compression efficiency is not affected for most frames.







% \jc{
% \begin{itemize}
%     \item how to integrate it in webrtc: same logical interface for video coding, packetization. replacing vp8
    
%     \item autoencoder highlight: entropy encoder, i-frame model, p-frame model
    
%     \item use of intel vino to reduce overhead
% \end{itemize}
% }



